Feature Inference Attack on Model Predictions in Vertical Federated Learning

Federated learning (FL) is an emerging paradigm for facilitating multiple organizations' data collaboration without revealing their private data to each other. Recently, vertical FL, where the participating organizations hold the same set of samples but with disjoint features and only one organization owns the labels, has received increased attention. This paper presents several feature inference attack methods to investigate the potential privacy leakages in the model prediction stage of vertical FL. The attack methods consider the most stringent setting that the adversary controls only the trained vertical FL model and the model predictions, relying on no background information. We first propose two specific attacks on the logistic regression (LR) and decision tree (DT) models, according to individual prediction output. We further design a general attack method based on multiple prediction outputs accumulated by the adversary to handle complex models, such as neural networks (NN) and random forest (RF) models. Experimental evaluations demonstrate the effectiveness of the proposed attacks and highlight the need for designing private mechanisms to protect the prediction outputs in vertical FL.

==> Vertical FL Attack Draft (arXiv final)/tex-files/revision.tex <==
\onecolumn

\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

\begin{auxmulticols}{2}

We would like to thank all the reviewers for their insightful and constructive comments. We have carefully addressed the comments, and have highlighted the major changes in the revised paper in {\color{blue} blue}.

\section*{Summary of Changes}
\label{sec-changes}

% \begin{itemize}
    % \item 
We have repeated the experiments relevant to Random Forest, changing the number of trees from 20 to 100, and implemented two new experiments for testing the impact of increasing query size with two real-world datasets. We added explanations and discussions on the questions raised in the review, and gave examples for each of the proposed methods.
% \end{itemize}

% \section*{Response to Meta-Reviewer}
% \noindent
% \textbf{Comment 1.} The reviewers liked the paper and would like to see a revision. Each reviewer lists a reasonably concrete list of suggestions. Please try to address them all.

% \vspace{2mm}\noindent
% \textbf{Response.} We have carefully addressed the comments point by point and revised the paper.

\section*{Response to Reviewer 1}
\noindent
\textbf{W1.} Some details of the proposed attacks need more explanations.

\noindent
\textbf{D1.} As W1 mentioned, how to approximately infer the features when $d_{target}\geq c$ in Sec.~IV-A? As most results in the experiments on equality solving attacks are in such case, please supplement the details of this part.

\vspace{2mm}\noindent
\textbf{Response.} We have refined the presentation in Section~\ref{subsec:attacks-lr-nn:specfic}. 
%
In particular, when $d_{\text{target}} \geq c$, the inference method is the same as that for $d_{\text{target}} \leq c -1$, i.e., $\hat{\boldsymbol{x}}_{\text{target}} = {\boldsymbol{\Theta}}_{\text{target}}^{+} \boldsymbol{a}$, where ${\boldsymbol{\Theta}}_{\text{target}}^{+}$ is the pseudo-inverse matrix of ${\boldsymbol{\Theta}}_{\text{target}}$. 
%
The rationale is that the solution based on the pseudo-inverse matrix not only minimizes the error norm $||\boldsymbol{\Theta}_{\text{target}} \hat{\boldsymbol{x}}_{\text{target}} - \boldsymbol{a}||_2$ but also minimizes the solution norm $||\hat{\boldsymbol{x}}_{\text{target}}||_2$, which provides a relatively good estimation, as demonstrated in our experiments. 
%
%In Section~\ref{subsec:experiments:individual}, we gave more explanations on the changes of the $\text{MSE}(\hat{\boldsymbol{x}}_{\text{target}}, \boldsymbol{x}_{\text{target}})$ under $d_{\text{target}} \geq c$.

\vspace{2mm}\noindent
\textbf{D2.} What is the time complexity of algorithm 1? Besides, what is the meaning of $\beta_{2k+1}$ and $\beta_{2k+2}$ in algorithm 1? Please clarify the details.

\vspace{2mm}\noindent
\textbf{Response.} We have added the time complexity analysis for Algorithm~\ref{alg:path-restriction}, and refined the presentation in Section~\ref{subsec:attack-dt}. 
%
The algorithm's time complexity is $O(n_f)$, where $n_f$ is the number of tree nodes in the full binary tree model. 
%
This is because the adversary needs to traverse the tree model to compute the indicator vectors for recording those tree nodes that may be evaluated in his perspective. 
%
Regarding $\beta_{2i+1}$ and $\beta_{2i+2}$ in the algorithm, they represent the corresponding indicators in $\boldsymbol{\beta}$ with respect to node $i$'s left and right child nodes, respectively. 
%
Specifically, an indicator value of 1 indicates that the node might be evaluated in this prediction in the perspective of the adversary; otherwise, the node will not be accessed (i.e., the prediction paths containing this node are impossible and can be eliminated). 

\vspace{2mm}\noindent
\textbf{W2.} The paper lacks of necessary examples to illustrate the proposed algorithms.

\noindent
\textbf{D3.} As W2 mentioned, though there is a simple example for path restriction attack, the algorithms would be more comprehensible if there are examples for the equality solving attack and attacks based on multiple predictions.

\vspace{2mm}\noindent
\textbf{Response.} As advised, to improve the presentation of the proposed attack methods, we have added two examples for the equality solving attack (Example~\ref{example:esa}) and generative regression network attack (Example~\ref{example:grna}) in Section~\ref{subsec:attacks-lr-nn:specfic} and Section~\ref{subsec:attacks-grn}, respectively.

\vspace{2mm}\noindent
\textbf{D4.} In Fig.~4, the increase of the MSE on datasets Bank marking and News popularity is much larger than that on Credit card and Drive diagnosis. In Fig.~5, the CBR of PRA increases slightly as $d_{\text{target}}$ increases, which contradicts the common sense and other instances. Please analyze the reasons.

\vspace{2mm}\noindent
\textbf{Response.} We have analyzed the reasons and added more explanations in Section~\ref{subsec:experiments:individual}. 
%
Regarding the phenomenon in Fig.~\ref{fig:esa-performance}, the root cause is from the different distributions of the four datasets. 
%
Based on the pseudo-inverse matrix inference method, we compute the upper bound of the MSE between the inferred solution $\hat{\boldsymbol{x}}_{\text{target}}$ and the ground-truth $\boldsymbol{x}_{\text{target}}$, i.e., $\text{MSE}(\hat{\boldsymbol{x}}_{\text{target}}, \boldsymbol{x}_{\text{target}})$, for the Bank, Credit, Drive, News datasets, which are 0.6, 0.14, 0.45, and 0.34, respectively. 
%
In general, a larger upper bound implies a lower attack accuracy that the adversary can achieve. This explains why the increase of the MSE on Bank is much larger than the other datasets. 
%
Besides, although the upper bound of Drive is larger than that of News, there are 11 classes for this dataset, i.e., the adversary can obtain 10 equations for the inference, which contains more information than that from News (i.e., 4 equations). Therefore, the MSE of Drive is smaller than that of News. 

In terms of the counter-intuitive CBR trend on the Drive dataset in Fig.~\ref{subfig:pra-drive}, there are two reasons. 
%
First, the Drive dataset has 11 classes, which is much more than those in other datasets (2 in Bank and Credit, 5 in News). As such, in Drive, each class corresponds to a smaller number of tree paths. 
%
Therefore, given one specific class, there exist only a small number of candidate prediction paths, which leads an improved CBR. In this case, the adversary would not gain a significant advantage by knowing more features. %may not facilitate further restrictions. 
%
Second, the decision tree model only selects informative features during training, which means that the increase of $d_{\text{target}}$ in Drive does not necessarily increase the number of unknown features in the tree, since some features may never be selected. As a consequence, a larger $d_{\text{target}}$ do not always decrease the CBR of the PRA attack. 

%First, there are more classes (11) in Drive than in other datasets (2 in Bank and Credit, 5 in News), which means in the Drive dataset, one class could correspond to less tree branches. The possible prediction paths of one specific class can be therefore greatly reduced, leading to a sufficiently good CBR. And more known features may not facilitate further restrictions. Second, the decision tree model does not include all the features. Due to the randomness of feature selection, the increase of $d_{\text{target}}$ (i.e. unknown features) does not necessarily decrease the number of known features selected in the tree model, which means larger $d_{\text{target}}$ in Drive may not decrease the CBR of the PRA attack. 

\vspace{2mm}\noindent
\textbf{D5.} What are the values of mean $\mu$ and standard deviation $\sigma$ used in the baseline random guess method? Please clarify.

\vspace{2mm}\noindent
\textbf{Response.} The mean and standard deviation of the Gaussian distribution in the random guess method are $\mu = 0.5$ and $\sigma = 0.25$, respectively. This ensures that at least 95\% of the generated samples are within $(0, 1)$. We have clarified the settings and added another random guess baseline according to the Uniform distribution $\boldsymbol{U}(0, 1)$ in Section~\ref{subsec:experiments:setup}.

\section*{Response to Reviewer 3}
\noindent
\textbf{D1.} Mitigation techniques are discussed and also evaluated to show their effects on presented attacks. However, I wonder why the authors did not at all mention differential privacy as one additional mitigation technique.

\vspace{2mm}\noindent
\textbf{Response.} We did not mention differential privacy (DP) since it is unsuitable in our setting. In particular, DP requires that any information from sensitive data should be released using a randomized function, such that even if we arbitrarily change a record in the function's input, the distribution of the function's output remains roughly the same. In our context, the sensitive data is an unlabelled record, and the function that releases information is a machine learning model that predicts the record's label. If we are to achieve DP, then we should inject noise into the model, such that even if we arbitrarily modifies the input record, the distribution of the model's output label is almost unchanged. In other words, the model should provide roughly the same prediction for any input record. This apparently renders the model useless. Therefore, DP is unsuitable for our problem. In the revised paper, we include the above discussion in Section~\ref{sec:defense}.

%Differential Privacy (DP) is employed for protecting individual's data privacy such that the probability of producing a given output is not highly dependent on whether a particular sample is included in the input dataset or not. Essentially, DP is more effective in protecting data privacy over multiple samples. However, in the prediction stage of vertical FL, the sample id should be known to all the parties, i.e., every party knows exactly the predicting sample, which does not satisfy the DP definition. In fact, how to incorporate DP into vertical FL models is still an open problem. Therefore, DP is not considered as a defense method in this paper. 
%(\textit{Is this explanation persuasive or reasonable? Do we need to add this explanation in the main text?})

\vspace{2mm}\noindent
\textbf{W2.} It is not clear why mean square error is chosen as the metric to evaluate attack performance.

\noindent
\textbf{D2.} Currently, the attack performance for ESA and GRNA is evaluated with the measurement of mean square error. According to equation (10) the effect is averaged over all features in the data set. However, I am not sure if this is the right approach for real-world scenarios: there I expect different features having different privacy levels. A brief discussion how the errors are distributed between different features would be helpful to further understand the attack's consequences. For example, target features that are strongly correlated with features the adversary knows would result in lower errors intuitively.



\vspace{2mm}\noindent
\textbf{Response.} Since the equality solving attack (ESA) and generative regression network attack (GRNA) are regression tasks, we use the mean square error (MSE) to measure their overall accuracy in reconstructing multiple target features.
We added more discussion regarding the impact of data correlation between the known features $\boldsymbol{x}_{\text{adv}}$ and the unknown features $\boldsymbol{x}_{\text{target}}$ on the attack performance in Section~\ref{subsec:experiments:multiple}. As demonstrated in Fig.~\ref{fig-corre}, we found that a stronger correlation would result in a higher attack accuracy. Therefore, in real-world scenarios, the adversary may exploit prior knowledge of attribute correlations to estimate the accuracy of his attacks. %further decide whether to believe the inferred feature values based on their correlations with the known feature values. 

\vspace{2mm}\noindent
\textbf{W1.} The evaluation with synthetic data is not very well motivated. I understand that the authors decided to use synthetic data to evaluate different numbers of predictions, however, it is not completely clear to me why this was not possible with real-world datasets (with reduced numbers in that case).

\vspace{2mm}\noindent
\textbf{Response.} As advised, we have added new experiments using two real-world datasets (i.e., Drive diagnosis and News popularity) to evaluate the impact of different query sizes on the attack performance. The results show a similar trend to those using synthetic datasets. We have updated Fig.~\ref{fig:grn-sample-size} and the corresponding descriptions in Section~\ref{subsec:experiments:multiple}.

\section*{Response to Reviewer 4}
\noindent
\textbf{D1.} The paper proposes a novel attack in the setting of vertical federated learning which has drawn significant attention recently. It begins with an intuitive logistic regression to demonstrate the feasibility of such an attack. Even though this paper focuses on federated learning, the proposed methodology is also applicable to the problem of model inversion for sensitive features such as [1]. It is necessary to compare with the approaches in those attacks and address the differences.

\noindent
[1] The Secret Revealer: Generative Model-Inversion Attacks Against Deep Neural Networks, CVPR, 2020

\vspace{2mm}\noindent
\textbf{Response.} The basic idea of [1] is similar in spirit to ours, as it also tries to infer sensitive features (i.e., pixels) based on known image patches and white-box models. However, the method in [1] has two major differences from our approach. First, the method in [1] requires pre-training on public images to obtain the general image distributions, whereas our approach does not rely on the prior data distribution of the target features. Second, [1] aims to recover the training samples, whereas our attack methods mainly focus on reconstructing the prediction samples. We have added discussions on [1] in Section~\ref{sec:related-work}.

\vspace{2mm}\noindent
\textbf{D2.} The threat model can be improved. The paper claims that their method requires no background information while the definition of “background” is not clear. If it includes everything even the name/type of those features, it makes the inferred results less threatening given that the attacker has no idea what those features represent.

\vspace{2mm}\noindent
\textbf{Response.} We have improved the presentation of the threat model in Section~\ref{subsec:problem:threat-model} and the corresponding descriptions in Sections~\ref{sec:introduction} and \ref{sec:related-work}. Specifically, we emphasize that the adversary does not have background information of the attack target's data distribution, but may know the unknown feature's name, type, and value range. This assumption is reasonable because, in practice, the active party in vertical federated learning often needs this information to explain and justify the trained model before deploying it into the production system. 

\vspace{2mm}\noindent
\textbf{D3.} In Section V, the paper develops multiple predictions attack based on the assumption that the candidate tree combinations are large and 100 trees can produce (40,100), approximately $1\times{10}^{28}$. However, in the evaluation, the maximum number of trees is 20 which makes it only (8,20) combinations, which is around $1\times{10}^{5}$. It will be more sensible to have the same number of trees as the assumption does.

\vspace{2mm}\noindent
\textbf{Response.} We have conducted new experiments using 100 trees for the random forest model and updated Fig.~\ref{fig:grna-performance} and Fig.~\ref{fig:grna-rf-performance-cbr}. The results are similar to the setting with 20 trees, which demonstrates the effectiveness of the proposed attack method. We have also revised the description of this setting in Section~\ref{subsec:experiments:setup}.

\vspace{2mm}\noindent
\textbf{D4.} In Fig.~3, it seems building the generative model with a random input $\boldsymbol{r}^t$ is not meaningful since it neither contributes to the back-propagation or is necessarily needed as a seed.

\vspace{2mm}\noindent
\textbf{Response.} We have added the explanation of the effect of random input $\boldsymbol{r}^t$ in Section~\ref{sec:attack-multiple-predictions}. In fact, the random vector $\boldsymbol{r}^t$ is an indispensable component of GRN. First, it acts as a regularizer, encouraging the generator to capture more randomness arising from $\boldsymbol{x}^t_{\text{adv}}$. Second, in different epochs, the $\boldsymbol{x}^t_{\text{adv}}$ of a specific sample can be concatenated with different $\boldsymbol{r}^t$ into different generator inputs, which derive various gradient directions during the back-propagation and thus lead to a better estimation of $\boldsymbol{x}^t_{\text{target}}$ with high probabilities. 
In the experiments, we found that a generator with random inputs can reduce the reconstruction error by $20\%$ compared to those without random inputs.
Due to space limitation, we include this set of experiments in the arXiv version of this paper. 

\vspace{2mm}\noindent
\textbf{D5.} The impact of query size is important to the problem of multiple predictions since they need to be done by multiple parties jointly in vertical federated learning, which is missing from the evaluation or discussion.

\vspace{2mm}\noindent
\textbf{Response.} The impact of query size, i.e., the number of predictions, is evaluated in Section~\ref{subsec:experiments:multiple}, as shown in Fig.~\ref{fig:grn-sample-size}. In the revised paper, we have added new experiments on two real-world datasets (i.e., drive diagnosis and news popularity) to illustrate its effect on the attack performance. The results show that attack accuracy could be improved when the adversary accumulates more prediction outputs, which is expected as the generator model can be trained more accurately given more predictions. We have revised the description in Section~\ref{subsec:experiments:multiple}.

\vspace{2mm}\noindent
\textbf{D6.} In Section VI, the baselines are built by random samples from Gaussian distribution without specification of mean and variance. Besides, the uniform distribution should be more suitable for a random baseline. This needs to be clarified as the samples are most likely to be drawn from the mean area in Gaussian distribution.

\vspace{2mm}\noindent
\textbf{Response.} We have clarified the Gaussian distribution setting in the experiments: the mean is 0.5 and the standard deviation is 0.25. This setting ensures that at least 95\% of the generated samples are within (0,1). In addition, we have added another random baseline with a uniform distribution $\boldsymbol{U}(0,1)$ and updated Fig.~\ref{fig:esa-performance}, Fig.~\ref{fig:grna-performance} and Fig.~\ref{fig:grn-sample-size} in Section~\ref{sec:experiments}. 
%The results show that the two random baselines achieve a similar performance, (\textit{explain the reason?}).

\vspace{2mm}\noindent
\textbf{Minors.} Page 2: using multiple prediction;
Page 11: this is the first work addresses this problem.

\vspace{2mm}\noindent
\textbf{Response.} We have corrected the mentioned grammar problems.

\end{auxmulticols}

\twocolumn

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-acknowledgements.tex <==
\section*{Acknowledgement}\label{sec:acknowledgements}

This work is supported by xxx.

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-attack-lr-nn.tex <==
\section{Attack Based on Individual Prediction}
\label{sec:attacks-individual-prediction}

In this section, we consider the attack problem in Eqn~(\ref{eq:attack-problem}) based on individual model prediction, which means the adversary can initiate an attack once obtaining the prediction output of a sample. 
%
Specifically, we present an equality solving attack on the logistic regression (LR) model and a path restriction attack on the decision tree (DT) model in Section \ref{subsec:attacks-lr-nn:specfic} and \ref{subsec:attack-dt}, respectively.
%propose two attacks on the logistic regression and neural networks models. We first consider a specific attack when a condition is satisfied in Section \ref{subsec:attacks-lr-nn:specfic}, and present a general attack in Section \ref{subsec:attacks-lr-nn:general}.

\subsection{Equality Solving Attack}
\label{subsec:attacks-lr-nn:specfic}

%For simplicity, we assume there are only two parties: $P_1$ is the active party and also the adversary, $P_2$ is the passive party and the attack target. The attack can be easily extended to the situation of multiple parties with collusion, since we can consider the colluding parties as a single active party and the other parties as a single passive party.

As described in Section~\ref{subsec:background:machine-learning}, the LR model prediction of sample $\boldsymbol{x}$ is computed by a deterministic function $f(\boldsymbol{x}, \boldsymbol{\theta})$, where $\boldsymbol{\theta}$ is the model parameters known to the active party (i.e., the adversary). Therefore, given the prediction output $\boldsymbol{v}$, the adversary $P_{\text{adv}}$ can construct a set of equations, from which $P_{\text{adv}}$ could infer the feature values held by $P_{\text{target}}$. We discuss the binary LR classification and multi-class LR classification separately.

%In the individual prediction case, all the knowledge the adversary obtains is the trained model $\boldsymbol{\theta}$, the prediction output $\boldsymbol{v}$ and his own feature values of an input sample, as described in Eqn.~(\ref{eq:attack-problem}). 
%
%We observe that when a specific condition is satisfied in the LR model, the target party's feature values can be recovered with a high accuracy.

\vspace{1mm}\noindent 
\textbf{Binary LR prediction.} 
We denote the model parameters as $\boldsymbol{\theta} = (\boldsymbol{\theta}_{\text{adv}}, \boldsymbol{\theta}_{\text{target}})$, where $\boldsymbol{\theta}_{\text{adv}}$ and $\boldsymbol{\theta}_{\text{target}}$ are the weights corresponding to the features owned by $P_{\text{adv}}$ and  $P_{\text{target}}$, respectively.
%
Let $\boldsymbol{v}$ be the prediction output of a given sample $\boldsymbol{x} = (\boldsymbol{x}_{\text{adv}}, \boldsymbol{x}_{\text{target}})$.
%To make a prediction given $\boldsymbol{x} = (\boldsymbol{x}_{\text{adv}}, \boldsymbol{x}_{\text{target}})$, each party can compute a partial sum, i.e., the inner product of her own feature values and the corresponding feature weights. 
%
%Then the parties run a secure protocol to obtain the prediction output $\boldsymbol{v}$.
%a confidence score, say $v_1$, representing the probability to be predicted as the first class. 
Note that for binary LR classification, there is only one meaningful confidence score in $\boldsymbol{v}$, e.g., $v_1$ for the first class, and that for the second class can be derived by $1-v_1$.
%
Given $v_1$ and the adversary's own feature values $\boldsymbol{x}_{\text{adv}}$, it is straightforward for $P_{\text{adv}}$ to create an equation with $\boldsymbol{x}_{\text{target}}$ as the variables, i.e.,
\begin{align}\label{eq:single-lr-equation}
    %\sigma(x_{21} \theta_{21} + \cdots + x_{2 d_2} \theta_{2 d_2}) & = v
    \sigma(\boldsymbol{x}_{\text{adv}} \cdot \boldsymbol{\theta}_{\text{adv}} + \boldsymbol{x}_{\text{target}} \cdot \boldsymbol{\theta}_{\text{target}}) = v_1
\end{align}
where $\sigma(\cdot)$ is the sigmoid function. Obviously, if there is only one unknown feature, i.e., $d_{\text{target}} = 1$, then the equation has only one solution, which means the unknown feature value $\boldsymbol{x}_{\text{target}}$ can be inferred precisely.
\par

\vspace{1mm}\noindent
\textbf{Multi-class LR prediction.}
For multi-class LR classification, as mentioned in Section \ref{subsec:background:machine-learning}, there are $c$ linear regression models. Let $\boldsymbol{\theta} = (\boldsymbol{\theta}^{(1)}, \cdots, \boldsymbol{\theta}^{(c)})$ be the parameters for these $c$ models, respectively.
%
%and let $v_1, \cdots, v_{c}$ denote the confidence scores, respectively. 
To initiate the feature inference attack, the adversary aims to construct the following linear equations for $k \in \{1,\cdots,c\}$.
\begin{align}\label{eq:lr-equation-system}
    \boldsymbol{x}_{\text{adv}} \cdot \boldsymbol{\theta}_{\text{adv}}^{(k)} & + \boldsymbol{x}_{\text{target}} \cdot \boldsymbol{\theta}_{\text{target}}^{(k)} = z_k %\nonumber \\
    %& \cdots  \\
    %\boldsymbol{x}_{\text{adv}} \cdot \boldsymbol{\theta}_{\text{adv}}^{(c)} & + \boldsymbol{x}_{\text{target}} \cdot \boldsymbol{\theta}_{\text{target}}^{(c)} = z_c \nonumber
\end{align}
where $z_k$ is the output of the $k$-th linear regression model.
However, $P_{\text{adv}}$ only knows the confidence score vector $\boldsymbol{v} = (v_1, \cdots, v_{c})$ such that 
\begin{align}
    \label{eq:softmax-function}
    v_k = \frac{\exp{(z_k)}}{\sum\nolimits_{k'}\exp{(z_{k'})}}.
\end{align}
Also, it is impossible for $P_{\text{adv}}$ to revert $z_1, \cdots, z_{c}$ from $v_1, \cdots, v_{c}$ because there are multiple solutions to Eqn~(\ref{eq:softmax-function}). 
%However, the adversary only knows $v_1, \cdots, v_{c}$ and there are multiple solutions for $z_1, \cdots, z_{c}$ given these confidence scores.
Nevertheless, we observe that an important correlation exists between two confidence scores. Specifically, we can transform Eqn~(\ref{eq:softmax-function}) into:
\begin{align}
    %\label{eq:softmax-conversion}
    %\ln v_k & = \ln (\exp(z_k)) - \ln (\sum\nolimits_{k'} \exp(z_{k'})) \\
   %\Leftrightarrow 
   \ln v_k & = z_k - \ln (\sum\nolimits_{k'} \exp(z_{k'})). \label{eq:softmax-conversion-2}
\end{align}
Note that the second term in the right hand of Eqn~(\ref{eq:softmax-conversion-2}) is the same for all $k \in \{1,\cdots,c\}$. As a result, $P_{\text{adv}}$ can subtract $\ln v_k$ by another confidence score, say $\ln v_{k'}$, obtaining:
\begin{align}
    \label{eq:subtraction}
    \ln v_k - \ln v_{k'} = z_k - z_{k'}.
\end{align}
This property allows $P_{\text{adv}}$ to obtain $c-1$ linear equations by subtracting two adjacent equations in Eqn~(\ref{eq:lr-equation-system}), i.e.,
\begin{align}
    \label{eq:converted-equations}
    %\boldsymbol{x}_{\text{adv}} (\boldsymbol{\theta}_{\text{adv}}^{(1)} - \boldsymbol{\theta}_{\text{adv}}^{(2)}) & + \boldsymbol{x}_{\text{target}} (\boldsymbol{\theta}_{\text{target}}^{(1)} - \boldsymbol{\theta}_{\text{target}}^{(2)}) = \ln \frac{v_1}{v_2} \nonumber \\
    %& \cdots  \\
        \boldsymbol{x}_{\text{adv}} (\boldsymbol{\theta}_{\text{adv}}^{(k)} - \boldsymbol{\theta}_{\text{adv}}^{(k+1)}) & + \boldsymbol{x}_{\text{target}} (\boldsymbol{\theta}_{\text{target}}^{(k)} - \boldsymbol{\theta}_{\text{target}}^{(k+1)}) = a_k'
\end{align}
where $a_k' = \ln v_k - \ln v_{k+1}$ and $k \in \{1,\cdots, c-1\}$. 
Consequently, if the number of unknown features $d_{\text{target}} \leq c-1$, then there will be only one solution for $\boldsymbol{x}_{\text{target}}$, which can be inferred exactly. 

\vspace{1mm}\noindent
\textbf{Attack method.}
Based on the discussion for both binary LR and multi-class LR, we observe that when a specific condition is satisfied, i.e., $d_{\text{target}} \leq c-1$, $P_{\text{adv}}$ can infer $\boldsymbol{x}_{\text{target}}$ precisely. 
%
Due to that Eqn~(\ref{eq:single-lr-equation}) and Eqn~(\ref{eq:converted-equations}) are linear equations, we can rewrite them into matrix form, i.e., $\boldsymbol{\Theta}_{\text{target}} \boldsymbol{x}_{\text{target}} = \boldsymbol{a}$, where the dimension of $\boldsymbol{\Theta}_{\text{target}}$ is $(c-1) \times d_{\text{target}}$, and $\boldsymbol{x}_{\text{target}}$ and $\boldsymbol{a}$ are column vectors with size $d_{\text{target}}$ and $c-1$, respectively.
%
In particular, for binary LR, $\boldsymbol{\Theta}_{\text{target}}$ equals to $\boldsymbol{\theta}_{\text{target}}$ and $\boldsymbol{a}$ is $\sigma^{-1}(v_1) - \boldsymbol{x}_{\text{adv}} \cdot \boldsymbol{\theta}_{\text{adv}}$. While for multi-class LR, $\boldsymbol{\Theta}_{\text{target}}$ is composed of $c-1$ vectors $\boldsymbol{\theta}_{\text{target}}^{(k)} - \boldsymbol{\theta}_{\text{target}}^{(k+1)}$ for $k \in \{1, \cdots, c-1\}$ and $\boldsymbol{a}$ is derived from Eqn~(\ref{eq:converted-equations}) by substituting the known values. 
%
Given this matrix representation, the adversary can solve the target feature values easily by $\hat{\boldsymbol{x}}_{\text{target}} = {\boldsymbol{\Theta}}_{\text{target}}^{+} \boldsymbol{a}$, where ${\boldsymbol{\Theta}}_{\text{target}}^{+}$ is the pseudo-inverse matrix \cite{pseudoinverse} of $\boldsymbol{\Theta}_{\text{target}}$. 
% 
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

When $d_{\text{target}} \geq c$, although there are infinite solutions to Eqn~(\ref{eq:converted-equations}), the solution $\hat{\boldsymbol{x}}_{\text{target}}$ constructed by ${\boldsymbol{\Theta}}_{\text{target}}^{+} \boldsymbol{a}$, which minimizes $||\boldsymbol{\Theta}_{\text{target}} \hat{\boldsymbol{x}}_{\text{target}} - \boldsymbol{a}||_2$ and satisfies $||\hat{\boldsymbol{x}}_{\text{target}}||_2\leq ||\boldsymbol{x}_{\text{target}}||_2$ for all solutions (we refer the interested readers to~\cite{pseudoinverse} for more details), can still give a good estimation of $\boldsymbol{x}_{\text{target}}$.
We will experimentally demonstrate this in Section~\ref{sec:experiments}.

\newtheorem{example}{Example}
\begin{example}\label{example:esa}
Suppose the Bank in Fig.~\ref{fig:vertical-fl-example} tries to infer a user's unknown feature values that belong to the FinTech company. To illustrate the equality solving attack, we assume that there are 3 classes and the trained model parameters are $\boldsymbol{\Theta} = \begin{bmatrix}
\small
\boldsymbol{\theta}^{(1)}\\
\boldsymbol{\theta}^{(2)}\\
\boldsymbol{\theta}^{(3)}
\end{bmatrix} = 
\begin{bmatrix}
\small
0.08 & 0.0002 & 0.0005 & 0.09\\
0.06 & 0.0005 & 0.0002 & 0.08\\
0.01 & 0.0001 & 0.0004 & 0.05
\end{bmatrix}$. Suppose there is an input sample $\boldsymbol{x} = (25, 2\text{K}, 8\text{K}, 3)$, and the predicted confidence score vector is $\boldsymbol{v} = (0.867, 0.084, 0.049)$. $P_{\text{adv}}$ has the former two feature values `age=25' and `income=2K'. Then, from Eqn~(\ref{eq:subtraction})-(\ref{eq:converted-equations}), he can compute $\boldsymbol{\theta}_{\text{adv}}^{(1)} - \boldsymbol{\theta}_{\text{adv}}^{(2)}= (0.02, -0.0003)$, $\boldsymbol{\theta}_{\text{adv}}^{(2)} - \boldsymbol{\theta}_{\text{adv}}^{(3)}= (0.05, 0.0004)$, $\boldsymbol{\theta}_{\text{target}}^{(1)} - \boldsymbol{\theta}_{\text{target}}^{(2)}= (0.0003, 0.01)$, $\boldsymbol{\theta}_{\text{target}}^{(2)} - \boldsymbol{\theta}_{\text{target}}^{(3)}= (-0.0002, 0.03)$, $a_1' = 2.334$, and $a_2' = 0.539$. Consequently, $P_{\text{adv}}$ can construct two equations and estimate $\hat{\boldsymbol{x}}_{\text{target}} = (8011.8, 3.046)$, where the loss is from the precision truncation during the computations.
\end{example}

% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }

%(need re-write) In summary, for both binary LR and multi-class LR models, $P_{\text{adv}}$ can infer $\boldsymbol{x}_{\text{target}}$ precisely. 
%
%Specifically, to compute $\boldsymbol{x}_{\text{target}}$, Eqn~(\ref{eq:single-lr-equation}) and Eqn~(\ref{eq:converted-equations}) can be rewritten into matrix form, i.e., $\boldsymbol{x}_{\text{target}} \cdot \boldsymbol{\Theta} = \boldsymbol{A}$, where the dimensions of $\boldsymbol{x}_{\text{target}}, \boldsymbol{\Theta}, \boldsymbol{A}$ are $(1 \times d_{\text{target}})$, $(d_{\text{target}} \times c-1)$, $(1 \times c-1)$, respectively. In binary LR, $\boldsymbol{\Theta}$ is $\boldsymbol{\theta}_{\text{target}}$ and $\boldsymbol{A}$ is $v_1$. 
%
%In multi-class LR, $\boldsymbol{\Theta}$ is composed of $c-1$ vectors $\boldsymbol{\theta}_{\text{target}}^{(k)} - \boldsymbol{\theta}_{\text{target}}^{(k+1)}$ for $k \in \{1, \cdots, c-1\}$ and $\boldsymbol{A}$ is a computed known vector (by substituting $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{\theta}_{\text{adv}}^{(1)}, \cdots, \boldsymbol{\theta}_{\text{adv}}^{(c)}$ in Eqn~(\ref{eq:converted-equations})). 
%
%After that, the adversary can infer the target feature values by $\boldsymbol{x}_{\text{target}} = \boldsymbol{A} {\boldsymbol{\Theta}}^{-1}$, where ${\boldsymbol{\Theta}}^{-1}$ is the pseudo-inverse matrix of $\boldsymbol{\Theta}$. 
%

%Specifically, the adversary can solve this linear equation system easily. We will show in Section \ref{sec:experiments} that this attack achieves an accurate inference when $d_{\text{target}} \leq c-1$ and a relatively high accuracy even when $d_{\text{target}} > c-1$.

%Eqn~(\ref{eq:converted-equations}) can be rewritten into matrix form: $\boldsymbol{x}_{\text{target}} \cdot \boldsymbol{\Theta}_{\text{target}} = \boldsymbol{z}$

%Similarly, in this case, if $d_2 \leq c$, then there is only one solution for the unknown variables $\boldsymbol{x}_{\text{target}}$, which means the adversary can infer $P_{\text{target}}$'s feature values in each prediction.

%%%wyc: remove as this does not hold
%\vspace{2mm}
%\noindent
%\textbf{Neural Networks (NN) Prediction.}
%This attack also happens in NN models. In a NN model, the number of confidence scores equals to the number of class labels $c$ in the output layer. Therefore, in the perspective of the adversary, if the number of unknown feature values of the target party $d_{\text{target}}$ is no larger than $c$, there should be only one solution and it can be inferred with a high accuracy.

\begin{comment}
\vspace{2mm}
\noindent
\textbf{Approximate Attack Method.} Instead of directly solving the non-linear equation systems, which might be difficult to compute, we use a learning-based algorithm to approximately estimate the unknown feature values of the target party.

\IncMargin{0.5em}
\begin{algorithm}[t]
\DontPrintSemicolon
\small
\KwIn{${\boldsymbol{x}_{\text{adv}}}$: adversary's feature values,
${\boldsymbol{\theta}}$: model parameters, %\newline
${\boldsymbol{v}}$: confidence scores,
$\alpha$: step size
}
\KwOut{$\boldsymbol{x}_{\text{target}}^*$: inferred feature values of the target party}
{
    $\boldsymbol{x}_{\text{target}}' \leftarrow \mathcal{N}(0,1) $ $\slash\slash$randomly sample feature values \\
    \While{exit conditions not satisfied} {
        $\boldsymbol{v}' \leftarrow f(\boldsymbol{x}_{\text{adv}} \cup \boldsymbol{x}_{\text{target}}', \boldsymbol{\theta})$ $\slash\slash$compute prediction \\
        $\ell \leftarrow \textbf{err}(\boldsymbol{v}, \boldsymbol{v}')$ $\slash\slash$compute loss \\
        $\boldsymbol{x}_{\text{target}}' \leftarrow \boldsymbol{x}_{\text{target}}' - \alpha \cdot \bigtriangledown_{\boldsymbol{x}_{\text{target}}'} \ell$ 
    }
    return $\boldsymbol{x}_{\text{target}}'$
}
\caption{Approximate Equality Solving Attack}\label{alg:specific-attack}
\end{algorithm}

Algorithm \ref{alg:specific-attack} describes the approximate attack method. 
%
The adversary first samples random values $\boldsymbol{x}_{\text{target}}'$ to initialize the unknown features. 
%
Then the adversary iteratively compute the prediction output $\boldsymbol{v}'$ (i.e., confidence scores) using $\boldsymbol{x}_{\text{target}}'$ and the public parameters $\boldsymbol{\theta}$ as well as his own feature values $\boldsymbol{x}_{\text{adv}}$. After that, the adversary can obtain the loss of $\boldsymbol{v}'$ and the ground-truth confidence scores $\boldsymbol{v}$. Next, $P_{\text{adv}}$ can update $\boldsymbol{x}_{\text{target}}'$ according to the gradients of the unknown features for a better estimation. The main loop can be stopped when some conditions are satisfied, e.g., reaching the maximum number of iterations or the loss of estimated confidence scores is less than a threshold. Finally, the estimation $\boldsymbol{x}_{\text{target}}^*$ can be obtained. 
%\textit{(Need to further analyze the attack accuracy of this method, is there only a global minima in NN model under this condition?)}
\end{comment}


\subsection{Path Restriction Attack}
\label{subsec:attack-dt}
For the DT model, the prediction output includes only the predicted class, with a confidence score of 1.
%
We propose a specific attack called \textit{path restriction attack}, by which the adversary can restrict the possible prediction paths in the tree model based on the predicted class and his own feature values. 

\begin{example}\label{example:pra}
Fig.~\ref{fig:path-restriction} illustrates the basic idea of this attack given Fig.~\ref{fig:vertical-fl-example}. The adversary $P_{\text{adv}}$ has partial feature values: `age=25' and `income=2K'. Then $P_{\text{adv}}$ can restrict the possible prediction paths from 5 (the total number of prediction paths) to 2 (with blue arrows).
%
Besides, if assuming that the predicted class of this sample is 1, $P_{\text{adv}}$ can identify the real prediction path (with red arrows) and correctly infer that $P_{\text{target}}$'s deposit feature value of this sample is larger than 5K. 
\end{example}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/fig-path-restriction-example.pdf}
\caption{Example of path restriction attack. Assume that $P_{\text{adv}}$'s feature values of an input sample is: `age=25' and `income=2K', while the predicted class is 1.}
%\vspace{-0.5cm}
\label{fig:path-restriction}
\end{figure}


Generally, let $n_p$ be the total number of prediction paths, the adversary can restrict the candidate prediction paths to $n_r$ paths by comparing his own feature values with the branching thresholds in the tree model and checking if the leaf label of a path matches the ground-truth predicted class. Consequently, for the inference, the adversary uniformly and randomly selects a path from the $n_r$ paths and checks the unknown feature values belong to which branch compared to the branching thresholds.

\begin{algorithm}[t]
\DontPrintSemicolon
\small
\KwIn{${\boldsymbol{x}_{\text{adv}}}$: adversary's feature values,
${\boldsymbol{\theta}}$: model parameters, %\newline
$k$: predicted class
}
\KwOut{
%$\{\boldsymbol{x}_{2t}^*\}_{t=1}^{n'}$: inferred feature values of target party, 
$\mathcal{P}$: possible prediction paths
}
{
    $\boldsymbol{\beta} = \boldsymbol{0}$ $\slash\slash$ initialize indicator vector  \\
    $Q \leftarrow $ root node (index 0) \\
    $\beta_0 = 1$ \\
    \While{$Q$ is not empty} {
        node $i$ $\leftarrow$ $Q.\textbf{pop}()$ \\
        \If{node $i$ belongs to the adversary} {
            \If{adversary's feature value $\leq$ threshold value} {
                $\beta_{2i+1} = \beta_i$, $\beta_{2i+2} = 0$
            }
            \Else{
                $\beta_{2i+1} = 0$, $\beta_{2i+2} = \beta_i$
            }
            %$\beta_{2i+1} = \textit{(go left branch)}$ ? $\beta_i$ : $0$ \\
            %$\beta_{2i+2} = \textit{(go left branch)}$ ? $0$ : $\beta_i$ 
        }
        \Else{
            $\beta_{2i+1} = \beta_{2i+2} = \beta_{i}$
        }
        \If{node $i$ is not leaf node}{
            $Q.\textbf{push}(2i+1)$, $Q.\textbf{push}(2i+2)$ \\
        }
    }
    $\boldsymbol{\alpha} \leftarrow$ compute the indicator vector, such that the elements of leaf nodes with label $k$ are set to 1 and otherwise 0 \\ 
    $\boldsymbol{\beta} \leftarrow$ element-wise multiplication of $\boldsymbol{\alpha}$ and $\boldsymbol{\beta}$ \\
    $\mathcal{P} \leftarrow$ find the paths that $\beta' = 1$ ($\forall \beta' \in \boldsymbol{\beta}$) \\
    return $\mathcal{P}$
}
\caption{Path restriction attack}\label{alg:path-restriction}
\end{algorithm}

% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

Algorithm \ref{alg:path-restriction} summarizes this attack method. 
Let $n_{f}$ be the number of tree nodes in the full binary tree. 
The adversary $P_{\text{adv}}$ first initializes an indicator vector $\boldsymbol{\beta}$ of size $n_f$ with 0 (line 1).
%
This vector is used for recording the tree nodes that may be evaluated in the perspective of $P_{\text{adv}}$.
%
Then $P_{\text{adv}}$ initializes a queue $Q$ with the root node (whose index is 0) and sets $\beta_0 = 1$ because the root node must be evaluated for any prediction (lines 2-3).
%
Next, $P_{\text{adv}}$ iteratively pops a node from $Q$ and checks the following conditions until $Q$ is empty (lines 4-14). 
%
If the feature on the current node belongs to $P_{\text{adv}}$, $P_{\text{adv}}$ updates the corresponding indicators of its child nodes in $\boldsymbol{\beta}$ according to the comparison result between his feature value and the branching threshold on that node (lines 6-10).
%
Otherwise, the indicators of the child nodes are the same as the indicator of the current node (line 12).
%
For example, in Fig.~\ref{fig:path-restriction}, given the branching condition `age=30' on the root node ($i = 0$) and the feature value `age=25' of the input sample, $P_{\text{adv}}$ can update $\beta_{2i+1} = \beta_i = 1$ and $\beta_{2i+2} = 0$ as the prediction goes into the left branch. 
%
After that, if the current node is not a leaf node, $P_{\text{adv}}$ pushes its child nodes into $Q$ for iteratively updating. 
%
As a result, $\boldsymbol{\beta}$ can be computed. For example, $\boldsymbol{\beta} = (1,1,0,1,1,0,0,1,0,0,0,0,0,0,0)$ given Fig.~\ref{fig:path-restriction}.
%
In the following, $P_{\text{adv}}$ computes another indicator vector $\boldsymbol{\alpha}$ with size $n_f$, such that the elements of leaf nodes with label $k$ are set to 1 and the others are set to 0 (line 15). 
%
For example, $\boldsymbol{\alpha} = (0,0,0,0,1,0,1,0,1,0,0,0,0,0,0)$ in Fig.~\ref{fig:path-restriction}.
%
Finally, $P_{\text{adv}}$ updates $\boldsymbol{\beta}$ by element-wise multiplication using $\boldsymbol{\alpha}$, and the restricted prediction paths are those elements with 1 in $\boldsymbol{\beta}$ (lines 16-17).
%
In Fig.~\ref{fig:path-restriction}, there is only one element is 1 (i.e., node index 4) in the updated $\boldsymbol{\beta}$, and the corresponding prediction path can be identified (i.e., with red arrows).
%
%\textit{As we will show in Section \ref{sec:experiments}, this attack has a high inference accuracy \textit{w.r.t.} the CBR metric comparing to the random guess inference.}
The complexity of Algorithm~\ref{alg:path-restriction} is $O(n_f)$ as the adversary needs to traverse the tree model to compute the indicator vectors.

% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }






==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-attack-trees.tex <==
\section{Attack Based on Multiple Predictions}\label{sec:attack-multiple-predictions}

So far, we identify two specific attacks based on individual model prediction. However, these attacks could hardly be applied to complex models, such as neural networks (NN) and random forest (RF).
%
%First, there is a specific condition on the number of unknown features in the equality solving attack, which might not be true in most cases. When this condition is not satisfied, there would be infinite solutions to the equations, leading to an inaccurate inference. 
For the NN model, there are a number of hidden layers for non-linear transformations, making it difficult to solve the equations by the equality solving attack. Even though the adversary could utilize the maximum a posteriori (MAP) method (e.g., \cite{fredrikson2015model}) to find a plausible solution, the attack accuracy would be undesirable because the solution space to the unknown features in the NN model is huge and irregular.
%
For the RF model, given the prediction output (i.e., the confidence scores), the number of candidate tree combinations might be too large. For example, if there are 100 trees in the RF model and a prediction output with two classes is $\boldsymbol{v} = (0.4,0.6)$, then the adversary needs to consider $C_{100}^{40}$ combinations of the trees, which is computationally expensive.

%Intuitively, we can also apply the path restriction attack as used for DT. For example, we can search the whole space to find all the possible prediction combinations of the trees. And restrict the combinations using the adversary's own feature values and $\boldsymbol{v}$. However, the space of candidate combinations may be too large, e.g., if $W=100$ and $\boldsymbol{v} = (0.4,0.6)$, then there are $C_{100}^{40}$ tree combinations, which is extremely computational expensive. 

%To address such problem, we propose to learn correlations between attacker's feature set $x_{adv}$ and targeting feature set  $x_{target}$ via a generative network in an unsupervised manner.
%We argue that correlations exist between $x_{adv}$ and $x_{target}$, or the models trained by vertical FL could not perform better than the local models trained respectively on $x_{adv}$ and $x_{target}$.



To address the above limitations, we design a general feature inference attack, called \textit{generative regression network} (GRN), based on multiple model predictions. 
%
The rationale that the adversary can rely on multiple predictions is that the active party can easily collect this information by observing model predictions of new samples in the long term, for example, in a week or a month, as long as the vertical FL model is unchanged.
%
These accumulated data could be used for initiating a more sophisticated inference attack. 
%As a result, the adversary can initiate this attack to backward infer the feature values of each sample. 

\begin{figure*}[t]
\centering
\includegraphics[width=0.75\textwidth]{figures/fig-generator-attack-illustration-new.pdf}
%\includesvg[width=0.7\textwidth]{figures/fig-generator-attack-illustration.svg}
\caption{Illustration of generative regression network trained by the adversary
%the goal is to train a generator model, whose output is the generated values of the unknown features, to minimize the total loss between the predicted outputs based on the generated samples and the ground-truth outputs.
}
\vspace{-0.5cm}
\label{fig:generator-attack-illustration}
\end{figure*}

Fig.~\ref{fig:generator-attack-illustration} gives an overview of this attack. The basic idea is to figure out the overall correlations between the adversary's own features and the attack target's unknown features. %based on the vertical FL model parameters $\boldsymbol{\theta}$, the prediction output $\boldsymbol{v}$, and the known feature values $\boldsymbol{x}_{\text{adv}}$. 
Upon this, the problem of inferring the unknown feature values is equivalent to the problem of generating new values $\hat{\boldsymbol{x}}_{\text{target}}$ to match the decisions of vertical FL model, where $\hat{\boldsymbol{x}}_{\text{target}}$ follows a probability distribution determined by the adversary's known feature values and the feature correlations.
To learn such a probability distribution, we build a generator model (in green color in Fig.~\ref{fig:generator-attack-illustration}) which takes the adversary's known feature values and a set of random variables as inputs (as depicted in the input layer in Fig.~\ref{fig:generator-attack-illustration}) and produces an estimation of the unknown feature values. The estimated values and the known feature values are combined into a \textit{generated sample}. 
Consequently, the generator model is trained by minimizing the loss between the predictions of the generated samples and the ground-truth predictions.
%

% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

\begin{example}\label{example:grna}
%Suppose the Bank in Fig.~\ref{fig:vertical-fl-example} aims to infer user $A$'s deposit and shopping information $\boldsymbol{x}^{(A)}_{\text{target}}=(\text{deposit}, \text{shopping})$ based on the 
Suppose that the Bank in Fig.~\ref{fig:vertical-fl-example} knows feature values $\boldsymbol{x}^t_{\text{adv}}=(\text{age }25, \text{income }2\text{K})$, and the prediction output $v^t=0.7$ if there are two classes. 
To infer the other two feature values, the Bank first feeds $\boldsymbol{x}^t_{\text{adv}}$ together with some random values $(25, 2\text{K}, r^t_1, r^t_2)$ into the generator to obtain a preliminary result, e.g. $\hat{\boldsymbol{x}}^t_{\text{target}}=(2\text{K}, 2)$;
then, $\boldsymbol{x}^t_{\text{adv}}$ and  $\hat{\boldsymbol{x}}^t_{\text{target}}$ are concatenated and input into the federated model to get a simulated output $\hat{v}^t=0.5$; 
the loss function $\ell(\hat{v}^t, v^t)$ is then calculated and back-propagated to the generator. 
With multiple predictions, the generator can learn the data distribution of the target features. %$\boldsymbol{P}(\boldsymbol{x}_{\text{target}} | \boldsymbol{x}_{\text{adv}}, v)$.
\end{example}

Note that the random vector $\boldsymbol{r}^t$ is an indispensable component of GRN. First, it acts as a regularizer, encouraging the generator to capture more randomness arising from $\boldsymbol{x}^t_{\text{adv}}$. Second, in different epochs, the $\boldsymbol{x}^t_{\text{adv}}$ of a specific sample can be concatenated with different $\boldsymbol{r}^t$ into different generator inputs, which derive various gradient directions during the back-propagation and thus lead to a better estimation of $\boldsymbol{x}^t_{\text{target}}$ with high probabilities. 
In Section~\ref{subsec:experiments:multiple}, we show that a generator with random inputs can reduce the reconstruction error by $20\%$ compared to those without random inputs.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }

Unlike existing feature inference attacks, our attack method considers the most stringent case: it relies on no intermediate information disclosed during the computation (required in~\cite{MelisSCS19, ZhuLH19, hitaj2017deep, wang2019beyond}) and no background information of the attack target's data distribution (such as statistics or marginal feature distribution required in~\cite{fredrikson2014privacy, fredrikson2015model, yeom2018privacy}). 
%
In particular, the adversary only needs a set of model predictions and the vertical FL model for initiating the attack. 
%distribution of the samples based on these prediction results and the adversary's own data. Specifically, the goal is to train a generator (i.e., a neural network model) that mimics the correlations between known features and unknown features.
In this section, we first present this attack on the NN model in Section~\ref{subsec:attacks-grn} and then describe how to extend it to the RF model in Section~\ref{subsec:attack-rf}.

\subsection{Generative Regression Network}
\label{subsec:attacks-grn}

%Recall that, there is a condition $d_2 \leq c-1$ in the specific attack, which means the number of the target party's features should be no more than $c-1$. Otherwise, there would be infinite solutions for the equation system. We now consider a general attack that does not rely on this condition. 

%Since in the prediction stage, the adversary can obtain the prediction results of a number of samples, the basic idea of this attack to learn the distribution of the samples based on these prediction results and the adversary's own data. Specifically, the goal is to train a generator (i.e., a neural network model) that mimics the correlations between known features and unknown features. 

We assume that the adversary $P_{\text{adv}}$ has collected prediction outputs of $n$ samples in $\mathcal{D}_{\text{pred}}$, where $\mathcal{D}_{\text{pred}} = (D_{\text{adv}}, D_{\text{target}})$ such that the $t$-th ($t \in \{1, \cdots, n\}$) sample is represented by $\boldsymbol{x}^{t} = (\boldsymbol{x}_{\text{adv}}^{t}, \boldsymbol{x}_{\text{target}}^{t})$. 
Let $V = (\boldsymbol{v}^1, \cdots, \boldsymbol{v}^{n})$ be the corresponding $n$ prediction outputs. 
%Fig.~\ref{fig:generator-attack-illustration} gives an overview of the generative regression network (GRN) training. 
The adversary's objective is to train a generator model, say $\boldsymbol{\theta}_G$, such that given the known feature values of the $t$-th sample $\boldsymbol{x}_{\text{adv}}^t$ and a random value vector $\boldsymbol{r}^t$ with size $d_{\text{target}}$, the generator outputs the corresponding estimation $\hat{\boldsymbol{x}}_{\text{target}}^t$ of the target party's $\boldsymbol{x}_{\text{target}}^t$.
%
To train the model, $P_{\text{adv}}$ can apply the mini-batch stochastic gradient descent method, where the training dataset is composed of $D_{\text{adv}}$ and $V$. 
The objective function is as follows:
\begin{align}
    \label{eq:generator-obj-func}
    \min_{\boldsymbol{\theta}_G} \frac{1}{n} \sum_{t=1}^{n} \ell (f(\boldsymbol{x}_{\text{adv}}^t, f_G(\boldsymbol{x}_{\text{adv}}^t, \boldsymbol{r}^t; \boldsymbol{\theta}_G); \boldsymbol{\theta}), \boldsymbol{v}^t) + \Omega(f_G)
\end{align}
where $\boldsymbol{\theta}$ and $\boldsymbol{\theta}_G$ are the parameters of the vertical FL model and the generator model, respectively. 
%
Moreover, $f_G$ denotes $\hat{\boldsymbol{x}}_{\text{target}}^t$, i.e., the output of the generator, and $f$ denotes the output of the vertical FL model given the generated sample (concatenated by $\boldsymbol{x}_{\text{adv}}^t$ and $\hat{\boldsymbol{x}}_{\text{target}}^t$). 
%
Besides, $\Omega(\cdot)$ is a regularization term of the generated unknown feature values $\{\hat{\boldsymbol{x}}_{\text{target}}^t\}_{t=1}^n$. For example, we penalize the generator model when the variance of $\{\hat{\boldsymbol{x}}_{\text{target}}^t\}_{t=1}^n$ is too large, preventing from generating meaningless samples. Nevertheless, the variance is computed based on the generated values, thus no prior information is needed by the adversary.


Algorithm~\ref{alg:generator-attack} presents the training method for GRN.
Specifically, in each iteration of each epoch, $P_{\text{adv}}$ first selects a batch of samples $B = (\boldsymbol{x}_{\text{adv}}^1, \cdots, \boldsymbol{x}_{\text{adv}}^{|B|})$ from $D_{\text{adv}}$ and initializes a set of $|B|$ random vectors $R = (\boldsymbol{r}^1, \cdots, \boldsymbol{r}^{|B|})$. The size of each random vector is the number of features held by the attack target $P_{\text{target}}$.
%
Then for the $t$-th sample in $B$, $P_{\text{adv}}$ feeds $\boldsymbol{x}_{\text{adv}}^t$ along with the corresponding $\boldsymbol{r}^t$ into the generator, obtaining $\hat{\boldsymbol{x}}_{\text{target}}^t$.
%
Next, $P_{\text{adv}}$ concats $\boldsymbol{x}_{\text{adv}}^t$ with $\hat{\boldsymbol{x}}_{\text{target}}^t$ to obtain a complete generated sample and makes a prediction using the vertical FL model, resulting in a prediction output $\hat{\boldsymbol{v}}^t$. 
%
As a result, the loss of this generated sample can be calculated by a loss function $\ell(\cdot, \cdot)$, e.g., MSE, with the ground-truth prediction output $\boldsymbol{v}^t$.
After obtaining the losses of all samples in $B$, the adversary back-propagates the aggregated loss to update the parameters of the generator model $\boldsymbol{\theta}_G$. 
Finally, the adversary can obtain the trained generator model after all the training epochs.


%%%wyc: comment out 20200909
%To optimize Eqn~(\ref{eq:generator-obj-func}), we can use stochastic gradient descent to train the model. Algorithm presents the attack method. First, we initialize the parameters of the $\boldsymbol{\theta}_g$ (line 1). Next, for each batch in each epoch, we initialize random values for the unknown features in the batch (say $R$ in line 4) and feed them into the generator along with known features. The generator outputs the generated unknown feature values (say $\hat{X}_{2t}$) that follow the underlying distribution of the joint datasets (line 5). 
%After that, we concat the known feature values with the generated unknown feature values to obtain the generated samples $(X_{1t}, \hat{X}_{2t})$.
%Then we use the trained VFL to compute the prediction output of these generated samples (i.e., $\hat{V}$ in line 6) and compute the loss $\ell$ using ground-truth confidence values $V$ (line 7). Finally, the loss is back-propagated to update the parameters of the generator (line 8).
%After all the epochs, we can obtain the estimated generator parameters $\boldsymbol{\theta}_g^*$. 
%As a result, for any input sample, we could use the generator to infer the unknown feature values of the target party. 


After obtaining $\boldsymbol{\theta}_G$, the adversary can use it to infer the unknown feature values $D_{\text{target}}$ in $\mathcal{D}_{\text{pred}}$. Specifically, for any sample $\boldsymbol{x}$ in $\mathcal{D}_{\text{pred}}$, the adversary generates a random vector $\boldsymbol{r}$ and directly computes $f_G(\boldsymbol{x}_{\text{adv}} \cup \boldsymbol{r}, \boldsymbol{\theta}_G)$ as the inferred feature values.
Notice that the samples to be attacked are exactly the samples for training the generator model.
This property ensures that the adversary can accumulate as many model predictions as possible to train the generator and improve the attack performance. We will experimentally show the effect of the number of model predictions in Section~\ref{sec:experiments}.

%There are two ways for the inference given a sample $\boldsymbol{x}_{\text{adv}}$ and its prediction output $\boldsymbol{v}$. 
%First, the adversary randomly generates a random vector $\boldsymbol{r}$ and directly computes $f_G(\boldsymbol{x}_{\text{adv}} \cup \boldsymbol{r}, \boldsymbol{\theta}_G)$ as the inferred values. 
%Second, the adversary randomly generates a set of random vectors, computes the corresponding generated samples using the generator model, and feeds them into the trained VFL model, obtaining a set of prediction outputs. Then the adversary selects top-$K$ generated samples whose prediction outputs are close to the ground-truth $\boldsymbol{v}$, and uses their median as the inferred values.

%for each sample $(\boldsymbol{x}_{\text{adv}}^t, \boldsymbol{x}_{\text{target}}^t)$ and its prediction output $\boldsymbol{v}^t$, the adversary can generate a set of random vectors $\boldsymbol{r}^t$

Fig.~\ref{fig:grn-explain} gives an intuitive explanation for the GRN attack. Suppose two parties collaboratively train a linear model $v=f(\theta_{\text{adv}} x_{\text{adv}}+ \theta_{\text{target}} x_{\text{target}})$. The black dashed line represents the decision boundary of $f$, and the green dashed line represents the domain of $\boldsymbol{x}=(x_{\text{adv}}, x_{\text{target}}) $ with confidence $v=0.7$. In the prediction 
stage, the adversary wishes to reconstruct the values of $x_{\text{target}}$ under $v=0.7$ based on the features $x_{\text{adv}}$ owned by himself and the model $f$. With $f$ and $v$, the possible domain of $x_{\text{target}}$ is reduced to the green dashed line. Then, according to the distribution of $x_{\text{adv}}$, GRN can infer the corresponding distribution of $x_{\text{target}}$ with high accuracy.

The GRN attack method is general because it takes the trained vertical FL model as a black-box, as long as that model's objective function is differentiable, such that the prediction loss could be back-propagated to the generator model. Thus, this attack works for both LR and NN models.
%We will discuss the situation when the trained VFL model is not differentiable shortly.
%(However, as the loss should be back-propagated through the trained VFL model to the generator, the objective function of the trained VFL model needs to be differentiable. As as result, the tree-based models do not satisfy this requirement, we will discuss how to address the tree-based models in Section \ref{sec:attack-trees}.)

\begin{figure}[b]
\centering
\includegraphics[width=.7\columnwidth]{figures/explain.pdf}
\caption{An intuitive explanation for Generative Regression Network attack}
%\vspace{-0.5cm}
\label{fig:grn-explain}
\end{figure}

\subsection{Adopt GRN Attack on the Random Forest Model}
\label{subsec:attack-rf}

Let $W$ be the number of trees in the RF model. When predicting a sample, each tree produces a predicted class. The prediction output $\boldsymbol{v} = (v_1, \cdots, v_c)$ represents the fraction of trees that predict a label for each class. 
As discussed at the beginning of this section, the path restriction attack (see Section~\ref{subsec:attack-dt}) does not apply to the RF model, especially when $W$ is large.
%Intuitively, we can also apply the path restriction attack as used for DT. For example, we can search the whole space to find all the possible prediction combinations of the trees. And restrict the combinations using the adversary's own feature values and $\boldsymbol{v}$. However, the space of candidate combinations may be too large, e.g., if $W=100$ and $\boldsymbol{v} = (0.4,0.6)$, then there are $C_{100}^{40}$ tree combinations, which is extremely computational expensive. 
Therefore, we desire to apply the GRN attack method on the RF model. However, since the objective function of the RF model is not differentiable, it is impossible to back-propagate the prediction loss through the RF model to the generator. 

To address this issue, we add an additional step in the attack method. After obtaining the vertical FL model (i.e., RF), the adversary can train another differentiable model (e.g., NN) to approximate the RF model~\cite{biau2019neural}. Specifically, the adversary first generates a number of dummy samples, say $D_{\text{dummy}}$ from the whole data space, then predicts each dummy sample by the RF model. Let $V_{\text{dummy}}$ be the prediction outputs. After that, the adversary could train an NN model $\boldsymbol{\theta}_{A}$ based on $(D_{\text{dummy}}, V_{\text{dummy}})$. 
Essentially, the NN model $\boldsymbol{\theta}_{A}$ is used to simulate the behavior of the RF model. 
As a consequence, the adversary can replace the RF model $\boldsymbol{\theta}$ with the new NN model $\boldsymbol{\theta}_{A}$ in Algorithm~\ref{alg:generator-attack} to train the generator model and infer the unknown feature values.

\begin{algorithm}[t]
\DontPrintSemicolon
\small
\KwIn{${\{\boldsymbol{x}_{\text{adv}}^t\}_{t=1}^{n}}$: adversary's feature values,
${\boldsymbol{\theta}}$: parameters of the vertical FL model, %\newline
${\{\boldsymbol{v}^t\}}_{t=1}^n$: confidence scores, $\alpha$: learning rate
}
\KwOut{
%$\{\boldsymbol{x}_{2t}^*\}_{t=1}^{n'}$: inferred feature values of target party, 
$\boldsymbol{\theta}_G^*$: parameters of the generator model
}
{
    $\boldsymbol{\theta}_G \leftarrow \mathcal{N}(0,1)$ $\slash\slash$initialize generator model parameters \\
    \For{each epoch} {
        \For{each batch}{
            $loss = 0$ \\
            $B \leftarrow$ randomly select a batch of samples \\
            ${R} \leftarrow \mathcal{N}(0,1)$ $\slash\slash$initialize batch random values \\
            \For{$t \in \{1, \cdots, |B|\}$}{      $\hat{\boldsymbol{x}}_{\text{target}}^t \leftarrow f_G(\boldsymbol{x}_{\text{adv}}^t \cup \boldsymbol{r}^t; \boldsymbol{\theta}_G)$ \\ 
            $\hat{\boldsymbol{v}}^t \leftarrow f(\boldsymbol{x}_{\text{adv}}^t \cup \hat{\boldsymbol{x}}_{\text{target}}^t; \boldsymbol{\theta})$ \\
            $loss$ += $\ell(\hat{\boldsymbol{v}}^t, {\boldsymbol{v}}^t)$ \\
            }
            $\boldsymbol{\theta}_G \leftarrow \boldsymbol{\theta}_G - \alpha \cdot \bigtriangledown_{\boldsymbol{\theta}_G} loss$ $\slash\slash$update parameters
        }
    }
    return $\boldsymbol{\theta}_G$
}
\caption{Generative regression network training}\label{alg:generator-attack}
\end{algorithm}

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-background.tex <==
\section{Preliminaries}\label{sec:background}

\subsection{Machine Learning} \label{subsec:background:machine-learning}
A machine learning (ML) model is a function $f(\boldsymbol{\theta}): \mathcal{X} \rightarrow \mathcal{Y}$ represented by a set of parameters $\boldsymbol{\theta}$, where $\mathcal{X}$ denotes the input (or feature) space, and $\mathcal{Y}$ the output space \cite{MelisSCS19}. 
%
In this paper, we focus on supervised classification learning, which builds a model from a labeled training dataset consisting of a set of samples. 
\par 

Given a training dataset $\mathcal{D}_{\text{train}}$ with $n$ samples $\boldsymbol{x}^t (t \in \{1, \cdots, n\})$ each containing $d$ features and the corresponding output label $y^t$, to learn the parameters $\boldsymbol{\theta}$, the training algorithm optimizes a loss function, i.e., 
%
\begin{align}\label{eq:loss-function}
    \min_{\boldsymbol{\theta}} \frac{1}{n} \sum_{t=1}^{n} \ell (f(\boldsymbol{x}^t, \boldsymbol{\theta}), y^t) + \Omega(\boldsymbol{\theta})
\end{align}
%
where $\ell(f(\boldsymbol{x}^t, \boldsymbol{\theta}), y^t)$ denotes the loss of sample $\boldsymbol{x}^t$ with label $y^t$, and $\Omega(\boldsymbol{\theta})$ is the regularization term that penalizes model complexity to avoid overfitting. 

%After the training is completed, we obtain the model parameters $\boldsymbol{\theta}$. As a result, given an input sample $\boldsymbol{x}$, the corresponding model prediction can be computed.
After obtaining the trained model parameters $\boldsymbol{\theta}$, we can compute the corresponding model prediction given any input sample $\boldsymbol{x}$.
%
In practice, the prediction output is composed of a vector of confidence scores, i.e., $\boldsymbol{v} = (v_1, \cdots, v_c)$, where each score represents the probability of $\boldsymbol{x}$ belonging to a class label, and $c$ is the number of classes.
%
Consequently, the classification is calculated by choosing the class label that has the highest confidence score.
\par

%\textbf{Stochastic Gradient Descent (SGD)}. To solve Eqn (\ref{eq:loss-function}), an effective and general algorithm is stochastic gradient descent (SGD), which approaches a local minimum of the loss function step by step. The SGD algorithm works as follows: $\textbf{w}$ is initialized as random values; in each iteration, a data point $(\textbf{x}_i, y_i)$ is selected randomly and $\textbf{w}$ is updated as 
%\begin{align}\label{eq:sgd-formula}
%    \textbf{w} := \textbf{w} - \alpha \frac{\partial \ell(f(\textbf{x}_i, \textbf{w}), y_i)}{\partial \textbf{w}}
%\end{align}
%where $\alpha$ is a learning rate defining the magnitude to move towards the minimum in each iteration. In practice, instead of selecting one data point per iteration, a small batch of samples are selected randomly and $\textbf{w}$ is updated by averaging the partial derivatives of all data points on the current $\textbf{w}$. We denote the set of indices selected in this mini-batch SGD method by $B$. \par

\vspace{1mm}\noindent
\textbf{Logistic regression (LR) model prediction.} 
%
In binary LR classification with two classes, the confidence score vector is $\boldsymbol{v} = (f(\boldsymbol{x}, \boldsymbol{\theta}), 1 - f(\boldsymbol{x}, \boldsymbol{\theta}))$, where
$f(\boldsymbol{x}, \boldsymbol{\theta}) = \sigma(\boldsymbol{\theta}^T \boldsymbol{x})$ and $\sigma(x) = (1 + e^{-x})^{-1}$, representing the probability that the input sample is classified into the first class.
%
In multi-class LR classification (i.e., $c > 2$), a typical method is multinomial classification, which trains a linear regression model $\boldsymbol{\theta}^{(k)}$ for each class $k \in \{1, \cdots, c\}$ and applies a softmax function on the $c$ linear regression predictions $f(\boldsymbol{x}, \boldsymbol{\theta}^{(1)}), \cdots, f(\boldsymbol{x}, \boldsymbol{\theta}^{(c)})$. 
%In classification where the number of classes $c > 2$, we can train $c$ binary LR models, in which one class is chosen as a \textit{pivot} and then the other $c-1$ classes are separately regressed against the pivot class. 
%
As a consequence, the output of the softmax function is the confidence score vector, i.e., the probabilities of the $c$ classes.
%In the prediction stage, the confidence scores are the output of the softmax function, i.e., the probabilities of the $c$ classes. 

\vspace{1mm}\noindent
\textbf{Neural networks (NN) model prediction}.
%
The neural network model is a popular architecture in deep learning. In an NN model, $f$ is typically composed of an input layer, an output layer, and a sequence of hidden layers with non-linear transformations from the input to the output. 
%
The model parameters $\boldsymbol{\theta}$ denote the weights for each transformation \cite{SongRS17}.
%
In the prediction stage, the results of the output layer are the confidence scores.
%
%Fig. \ref{fig:neural-network-example} shows a typical NN model with two hidden layers. 
%
%Each node represents a neuron, which is an instance of regression and is associated with an activation function. 
%
%Each connection between layers has a floating-point weight matrix as parameters. 
%
%These weights are updated by backward propagation during training \cite{Shokri15, Mohassel17, Melis19}. 
% 
%In the prediction stage, a forward computation is executed given an input sample, and the output layer gives the probabilities that the sample belongs to the possible classes.

%\begin{figure}[t]
%\centering
%\includegraphics[width=0.65\columnwidth]{figures/fig-neural-network-example.pdf}
%\caption{A neural network with two hidden layers. Black circles represent the bias node. Matrices $W_k$ contain the weights used in computing the activation functions at each layer $k$.}
%\label{fig:neural-network-example}
%\end{figure}

\vspace{1mm}\noindent
\textbf{Tree-based model prediction.} 
%
The decision tree (DT) model is widely adopted in real-world applications due to their good interpretability.
%
The DT model consists of a number of internal nodes and leaf nodes.
%
Each internal node describes a branching threshold \textit{w.r.t.} a feature, while each leaf node represents a class label.
%
When predicting an input sample, a sequence of branching operations are executed based on comparisons of the sample's feature values and the thresholds, until a leaf node is reached. 
%
The prediction output is the class label on that leaf node. Note that the branching operations are deterministic in the DT model. Therefore, the confidence score for the predicted class is 1, while the confidence scores for other classes are 0.

We can use ensemble models to further improve predictive performance, e.g., random forest (RF). 
%
Essentially, the RF model is composed of a set of independent DT models.
%
In the prediction stage, each tree predicts a class label, and the final classification is calculated by majority voting from all trees.
%
As a result, the prediction output of the RF model also includes a vector of confidence scores, where each element $v_k$ of class $k \in \{1, \cdots, c\}$ is the fraction of trees that predict $k$.

\subsection{Vertical Federated Learning} \label{subsec:vertical-federated-learning}

Vertical FL enables an active party (e.g., the bank in Fig.~\ref{fig:vertical-fl-example}) to enrich his business data by incorporating more diverse features of users from one or several passive parties (e.g., the Fintech company in Fig~\ref{fig:vertical-fl-example}). 
%
From which the active party could improve his model accuracy to provide better customer service. Meanwhile, the passive parties could benefit from a pay-per-use model \cite{WuZPM16} for their contributions to the model training and model prediction stages. 
%
For example, the active party may pay the passive parties according to the importance of their provided features \cite{simcollaborative}. 
%

In the prediction stage of vertical FL, a model prediction is usually initiated by the active party who sends a prediction request to other parties, along with an input sample id (e.g., 100 or 102 in Fig.~\ref{fig:vertical-fl-example}). 
%
The passive parties then prepare the corresponding feature values of that sample, and all parties jointly run a protocol to compute the prediction output. 
%
The protocol can be secure enough to protect each party's sensitive data, such that only the prediction output is revealed to the active party for making further decisions, and no intermediate information during the computation is disclosed~\cite{WuCXCO20}.

%secure multiparty computation protocol (e.g., \cite{WuCXCO20}) to compute the prediction output such that no intermediate information is disclosed (i.e., protecting each party's sensitive data). The prediction output would be revealed to the active party for making further decisions. 

%To protect each party's sensitive data and ensure that no intermediate information is disclosed during the model training and model prediction stages, the parties can utilize cryptographic techniques to provide strong security guarantees \cite{WuCXCO20}. Nevertheless, the trained vertical FL model and the model predictions (i.e., the confidence scores) are essential for the active party to make correct and interpretable decisions.  

%Federated learning (FL) is an emerging paradigm that enables multiple parties to jointly train a model without revealing their private data to each other.
%
%In this paper, we consider the vertical FL scenario, where each party holds a subset of the features while only one party, i.e., \textit{active party} owns the label information. The other parties are called \textit{passive parties}.
%
%For example, in digital banking, a bank and a Fintech company aim to jointly build an ML model that evaluates credit card applications.
%
%The bank has some partial information about the users (e.g., account balances), while the Fintech company has some other information (e.g., the users' online transactions). Also, only the bank has some historical evaluations about the users, i.e., labels.
%
%Specifically, the trained model is revealed to the participating parties for evaluating new applications.

%In this paper, we focus on the prediction stage, where the participating parties have already obtained the trained model and use it for serving new requests. The prediction output of a new input sample will be revealed to the active party (e.g., the bank) for making decisions.
%
%The active party could benefit from the more accurate decisions while the passive parties could benefit from a pay-per-use model \cite{WuZPM16} for its contribution to the prediction. 


%Let the number of parties be $m$ and the number of total features be $d$. 
%
%The number of features owned by party $P_i (i \in \{1,\cdots,m\})$ is denoted by $d_i$ while $\sum_{i=1}^m d_i = d$. 
%
%Without loss of generality, we assume that $P_1$ is the active party. 


==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

We present two specific attacks based on individual prediction output: equality solving and path restriction, for logistic regression and decision tree models, respectively. Furthermore, we design a general attack based on multiple prediction outputs for neural networks and random forest models. To our knowledge, this is the first work that investigates the privacy leakages in vertical FL. The experimental results demonstrate the accuracy of the proposed attacks and highlight the need for designing private algorithms to protect the prediction outputs. 

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-defense.tex <==
\section{Countermeasures}\label{sec:defense}

In this section, we discuss several potential defense methods that may mitigate the proposed feature inference attacks.

\vspace{1mm}\noindent
\textbf{Rounding confidence scores.}
In ESA, the adversary relies on the exact linear equations for the inference. Thus, a possible defense to ESA is to coarsen the confidence scores $\boldsymbol{v}$ returned to the active party, for example, round $\boldsymbol{v}$ down to $b$ floating point digits before revealing it.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }
Since the performances of the two random guess methods are similar, we only include the random guess with uniform distribution in this set of experiments.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }

Fig.~\ref{subfig:bank-conf-esa}-\ref{subfig:drive-conf-esa} show the effect of this strategy on two datasets, respectively.
We can observe that when rounding to 0.1 (i.e., $b=1$), the MSE per feature is higher than the random guess method, and the result is relatively stochastic. This is because that the equation result in Eqn~(\ref{eq:single-lr-equation}) or~(\ref{eq:converted-equations}) is related to $\ln \boldsymbol{v}$, a change of $\boldsymbol{v}$ with respect to 0.1 has thus a big impact on that result, leading to an inaccurate inference. In contrast, rounding to 0.001 (i.e., $b=3$) only has a small impact because the result would be mainly determined by the former three floating point digits.
%The parties can round the precision of confidence values to mitigate these attacks, for example, they can coarsen the precision of the exact output by 10\% before revealing it.
Fig.~\ref{subfig:bank-conf-grn}-\ref{subfig:drive-conf-grn} show the effect of the rounding strategy in GRNA for the LR model.
The results illustrate that GRNA is insensitive to the rounding of confidence scores, and the adversary can obtain a similar performance comparing to that without rounding. The reason is that GRNA learns the overall correlation between the adversary's features and the attack target's features, and the low-precision prediction outputs still indicate this pattern.

\vspace{1mm}\noindent
\textbf{Dropout for neural networks model.} Overfitting is considered to be an important factor in several inference attacks in the training stage \cite{ShokriSSS17, NasrSH2019}, as the trained model may memorize some underlying information of the data. We utilize a state-of-the-art regularization technique called dropout \cite{SrivastavaHKSS14} for training the vertical NN model to avoid overfitting. As depicted in Fig.~\ref{subfig:credit-dropout-grn}-\ref{subfig:news-dropout-grn}, using dropout slightly leads to a higher MSE per feature (i.e., degrade the attack performance), because dropout encourages NN models to memorize less distribution information of underlying datasets. Nevertheless, the adversary can still have a good inference because the generator model learns the overall feature correlations.


\vspace{1mm}\noindent
\textbf{Pre-processing before collaboration.}
Based on the experimental results in Section~\ref{sec:experiments}, we observe that:
(i) if the number of classes is relatively large, ESA can precisely recover the attack target's feature values, and PRA can correctly infer most branches in the tree model; (ii) if the adversary's features are highly correlated with the attack target's features, the attack performance of GRNA could be greatly improved.
%The attack performance of GRNA could be improved if $P_{\text{adv}}$ accumulates many prediction outputs or $P_{\text{adv}}$'s features are highly correlated with the attack target's features.
These observations inspire the parties to execute a pre-processing step that mitigates the potential privacy risks before data collaboration.
%, which is incorporated into our \textit{Falcon}\textsuperscript{\ref{note:falcon}} system.
%provide several useful insights on protecting model predictions in vertical FL collaboration:
First, the parties check the relationship between the number of classes and the number of their contributed features, ensuring no obvious privacy vulnerabilities.
Second, the parties collaboratively execute a secure protocol (e.g., using secure multiparty computation \cite{WuCXCO20}) to compute their feature correlations and remove those closely related features.
%(iii) the passive parties should be vigilant if the active party has requested a lot of predictions using the same trained model, as from which the active party may initiate a more powerful attack.

\vspace{1mm}\noindent
\textbf{Post-processing for verification.} The parties can also execute an additional verification step to check if the prediction output would lead to privacy leakage before revealing to the active party.
%For each model prediction request, after the parties jointly computing a prediction output using cryptographic techniques, they can execute an additional verification step to check if the result would cause privacy leakage before revealing the result to the active party.
For example, if the parties utilize secure hardware, e.g., Intel SGX, for computing the model predictions, then they can mimic these attacks inside the secure enclaves. Specifically, if the possible leakage exceeds a pre-defined threshold for any party, they do not reveal the prediction output for privacy protection.
%Essentially, the additional verification mimics these attacks against each party and only releases the prediction output when it satisfies the privacy of all parties.
%This step can be done using secure hardware, e.g., Intel SGX.
In other words, the prediction output is released only when it satisfies the privacy of all parties.
However, this post-processing step may incur huge overheads to the computation of model predictions.

\vspace{1mm}\noindent
\textbf{Hide the vertical FL model.}
Another consideration is to hide the trained vertical FL model using ciphertexts or secure multiparty computation compatible values, such that the adversary does not have access to the plaintext model in the attack.
%
This method could mitigate these attacks, but the active party cannot justify if the trained model is reasonable or not and cannot have a good interpretation of the prediction output for making important decisions.
%
A possible alternative is to use explainable predictions instead of revealing the trained vertical FL model, such that the contribution of each feature is provided to the active party for justification. However, it is still an open problem whether those explainable predictions would cause new privacy leakages.

%{\color{red} Differential Privacy (DP) is widely employed for privacy protection in horizontal FL. Specifically, DP, typically achieved by adding noises with a certain intensity to the shared data, can guarantee that the distributions of the uploaded gradients are not affected by the change of a single sample included in the training dataset. While in vertical FL, the entries of the shared model outputs correspond to the training samples. To achieve DP, i.e. to make any two shared entries indistinguishable, noises with relatively large intensities could be added, leading to unacceptable performance degradation of the federated model. Therefore, in vertical FL, DP is generally not the option for protecting data privacy, which is also not considered as a defense method in this paper.}

% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }



\vspace{2mm}\noindent
\textbf{Differential Privacy (DP).} DP~\cite{XiaoWG10} is a state-of-the-art privacy protection tool. However, it is unsuitable in our setting.
%
In particular, DP requires that any information from sensitive data should be released using a randomized function, such that even if we arbitrarily change a record in the function's input, the distribution of the function's output remains roughly the same.
%
In our context, the sensitive data is an unlabelled record, and the function that releases information is a machine learning model that predicts the record's label.
%
If we are to achieve DP, then we should inject noise into the model, such that even if we arbitrarily modifies the input record, the distribution of the model's output label is almost unchanged.
%
In other words, the model should provide roughly the same prediction for any input record.
%
This apparently renders the model useless. Therefore, DP is unsuitable for our problem.

% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }


==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-experiments.tex <==
\section{Experimental Evaluation}\label{sec:experiments}

This section shows the experimental evaluation of the proposed attacks. Section~\ref{subsec:experiments:setup} presents the experimental setup. The evaluations of the attacks based on individual model prediction and multiple model predictions are described in
Section~\ref{subsec:experiments:individual} and~\ref{subsec:experiments:multiple}, respectively.

\begin{figure*}[t]
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-bank-esa.pdf}
  %\vspace{-2mm}
  \caption{Bank marketing}
  \label{subfig:esa-bank}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-credit-esa.pdf}
  %\vspace{-2mm}
  \caption{Credit card}
  \label{subfig:esa-credit}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-drive-esa.pdf}
  %\vspace{-2mm}
  \caption{Drive diagnosis}
  \label{subfig:esa-drive}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-news-esa.pdf}
  %\vspace{-2mm}
  \caption{News popularity}
  \label{subfig:esa-news}
\end{subfigure}

\caption{Evaluation of equality solving attack \textit{w.r.t.} MSE per feature}
\vspace{-0.3cm}
\label{fig:esa-performance}
%\vspace{2mm}
\end{figure*}


\begin{figure*}[t]
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-bank-pra.pdf}
  %\vspace{-2mm}
  \caption{Bank marketing}
  \label{subfig:pra-bank}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-credit-pra.pdf}
  %\vspace{-2mm}
  \caption{Credit card}
  \label{subfig:pra-credit}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-drive-pra.pdf}
  %\vspace{-2mm}
  \caption{Drive diagnosis}
  \label{subfig:pra-drive}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-news-pra.pdf}
  %\vspace{-2mm}
  \caption{News popularity}
  \label{subfig:pra-news}
\end{subfigure}
%\vspace{-5mm}
\caption{Evaluation of path restriction attack \textit{w.r.t.} CBR}
\vspace{-0.3cm}
\label{fig:pra-performance}
%\vspace{2mm}
\end{figure*}

\subsection{Experimental Setup} \label{subsec:experiments:setup}

We implement the proposed attack algorithms in Python and conduct experiments on machines that are equipped with Intel (R) Xeon (R) CPU E5-1650 v3 @ 3.50GHz$\times$12 and 32GB RAM, running Ubuntu 16.04 LTS. Specifically, we adopt \textit{PyTorch}\footnote{\url{https://pytorch.org/}}  for training logistic regression (LR) and neural networks (NN) models, and \textit{sklearn}\footnote{\url{https://scikit-learn.org/stable/}} for training decision tree (DT) and random forest (RF) models.

\vspace{1mm}\noindent
\textbf{Datasets.} We evaluate the attack performance on four real-world datasets:
(i) bank marketing dataset \cite{MoroCR14}, which consists of 45211 samples with 20 features and 2 classes;
(ii) credit card dataset \cite{YehL09a}, which consists of 30000 samples with 23 features and 2 classes;
(iii) drive diagnosis dataset \cite{Dua2019}, which consists of 58509 samples with 48 features and 11 classes.
(iv) news popularity dataset \cite{FernandesV015}, which consists of 39797 samples with 59 features and 5 classes.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

Besides, we generate two synthetic datasets with the \textit{sklearn} library for evaluating the impact of the number of samples $n$ in the prediction dataset on the performance of generative regression network attack.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }
The first synthetic dataset includes 100000 samples with 25 features and 10 classes, and the second includes 100000 samples with 50 features and 5 classes.
We summarize the evaluated datasets in Table~\ref{tab-datasets}.
In addition, we normalize the ranges of all feature values in each dataset into $(0, 1)$ before training the models.

\begin{table}[t]
\caption{Statistics of Datasets}
\centering
\begin{tabular}{  c  c c c }
\toprule
Dataset & Sample Num. & Class Num. & Feature Num. \\
\toprule
Bank marketing &	45211&	2&	20\\
Credit card	&30000&	2	&23\\
Drive diagnosis	&58509&	11&	48\\
News popularity	&39797&	5&	59\\
Synthetic dataset 1	& 100000 &	10&	25\\
Synthetic dataset 2	& 100000 &	5&	50\\
\bottomrule
\end{tabular}
\label{tab-datasets}
\end{table}

\vspace{1mm}
\noindent
\textbf{Models.} We generate the vertical FL models using centralized training and give the trained models to the adversary. This is reasonable because we consider the case that no intermediate information is disclosed during the training process, and only the final model is released. We evaluate the attack performance on the four models discussed in this paper. By default, the maximum tree depth of the DT model is set to 5. For the RF model, the number of trees and the maximum tree depth are set to 100 and 3, respectively. Besides, the NN model is composed of an input layer (whose size equals to the number of total features $d$), an output layer (whose size equals to the number of classes $c$), and three hidden layers (with 600, 300, 100 neurons, respectively).

\vspace{1mm}
\noindent
\textbf{Metrics.} We evaluate the attack performance with two metrics.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

Since the equality solving attack (ESA) and generative regression network attack (GRNA) are regression tasks, we use the mean square error (MSE) per feature to measure their overall accuracy in reconstructing multiple target features.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }

Specifically, the MSE per feature is calculated as:
%by the deviation of the inferred feature values from the ground-truth and the division of the number of target features, i.e.,
\begin{align}
    \label{eq:mse-per-feature}
    \text{MSE} = \frac{1}{n * d_{\text{target}}} \sum\nolimits_{t=1}^n \sum\nolimits_{i=1}^{d_{\text{target}}} {(\hat{x}_{\text{target},i}^t - x_{\text{target},i}^t)}^2
\end{align}
where $n$ is the number of samples in the prediction dataset, $d_{\text{target}}$ is the number of target features, $\hat{\boldsymbol{x}}_{\text{target}}^t$ and $\boldsymbol{x}_{\text{target}}^t$ are the inferred feature values and the ground-truth of the $t$-th sample, respectively.
%
For the path restriction attack (PRA), we measure the correct branching rate (CBR). Specifically, we first randomly select a path from all the possible prediction paths computed by PRA, then accordingly measure the fraction of inferred feature values that belong to the correct branches (i.e., comparing to the ground-truth).
%
For each experiment, we conduct 10 independent trials and report the average result.

\vspace{1mm}
\noindent
\textbf{Baselines.} For ESA and GRNA,
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }
we use two baselines that randomly generate samples from $(0,1)$ according to a Uniform distribution $\boldsymbol{U}(0, 1)$ and a Gaussian distribution $\boldsymbol{N}(0.5, 0.25^2)$. This Gaussian distribution can ensure that at least $95\%$ samples are within $(0, 1)$.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }
For PRA on the DT model, we adopt a baseline that randomly selects a prediction path and evaluates CBR along that path. Both baselines are called \textit{random guess} in the following presentation.

\subsection{Evaluation of Attacks Based on Individual Prediction} \label{subsec:experiments:individual}

\begin{figure*}[t]
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-bank-grn-mse.pdf}
  %\vspace{-2mm}
  \caption{Bank marketing}
  \label{subfig:grna-bank}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-credit-grn-mse.pdf}
  %\vspace{-2mm}
  \caption{Credit card}
  \label{subfig:grna-credit}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-drive-grn-mse.pdf}
  %\vspace{-2mm}
  \caption{Drive diagnosis}
  \label{subfig:grna-drive}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-news-grn-mse.pdf}
  %\vspace{-2mm}
  \caption{News popularity}
  \label{subfig:grna-news}
\end{subfigure}

\caption{Evaluation of generative regression network attack \textit{w.r.t.} MSE per feature}
\vspace{-0.5cm}
\label{fig:grna-performance}
%\vspace{2mm}
\end{figure*}

For ESA and PRA based on individual model prediction (see Section~\ref{sec:attacks-individual-prediction}), we evaluate the attack performance \textit{w.r.t.} the number of features $d_{\text{target}}$ owned by the attack target $P_{\text{target}}$. In particular, we vary the fraction of $d_{\text{target}}$ (i.e., over the number of total features $d$) by $\{10\%, 20\%, 30\%, 40\%, 50\%, 60\%\}$.

\vspace{1mm}\noindent
\textbf{Effect of $d_{\text{target}}$ on ESA.} Fig.~\ref{fig:esa-performance} shows the attack performance of ESA \textit{w.r.t.} MSE per feature. For all the datasets, if the threshold condition $d_{\text{target}} \leq c - 1$ is satisfied (denoted by `T' in each sub-figure), the MSE per feature is 0. This is in line with what we have discussed in Section~\ref{subsec:attacks-lr-nn:specfic}. For example, there are 11 classes in the drive diagnosis dataset; thus in Fig.~\ref{subfig:esa-drive}, the unknown feature values can be precisely inferred when $d_{\text{target}} = 10$ (i.e., 20\% in percentage).

Moreover, we observe that even if the threshold condition is not satisfied, ESA can still find a good inference of $\boldsymbol{x}_{\text{target}}$, which is greatly superior to the random guess methods (e.g., in Fig.~\ref{subfig:esa-credit} and \ref{subfig:esa-drive}).
%
Besides, the MSE per feature increases as the fraction of $d_{\text{target}}$ increases. This is expected since the larger $d_{\text{target}}$ is, the more unknown variables in the equations, making the estimation more biased.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

In particular, the MSE increase of the Bank dataset is much larger than those of other datasets, which can be explained by the difference of data distributions of different datasets.
%
As mentioned in Section~\ref{subsec:attacks-lr-nn:specfic}, the solution $\hat{\boldsymbol{x}}_{\text{target}}$ computed by the pseudo-inverse matrix has the minimum Euclidean norm among all solutions, i.e., $||\hat{\boldsymbol{x}}_{\text{target}}||_2\leq ||\boldsymbol{x}_{\text{target}}||_2$, which indicates
\begin{equation}\label{eq-l2norm}
    \sum^{d_{\text{target}}}_{i=1} \hat{x}_{\text{target}, i}^2\leq \sum^{d_{\text{target}}}_{i=1} x_{\text{target}, i}^2.
\end{equation}
Accordingly, we have
\begin{align}
\text{MSE}&=\frac{1}{d_{\text{target}}}\sum^{d_{\text{target}}}_{i=1} (\hat{x}_{\text{target}, i} - {x}_{\text{target}, i})^2\\
       &=\frac{1}{d_{\text{target}}}\sum^{d_{\text{target}}}_{i=1} (\hat{x}_{\text{target}, i}^2 + {x}_{\text{target}, i}^2 - 2\hat{x}_{\text{target}, i}x_{\text{target}, i})\label{eq-base}\\
       &\leq\frac{1}{d_{\text{target}}}\sum^{d_{\text{target}}}_{i=1} (\hat{x}_{\text{target}, i}^2 + {x}_{\text{target}, i}^2) \label{eq-step1}\\
       &\leq\frac{1}{d_{\text{target}}}\sum^{d_{\text{target}}}_{i=1} 2{x}_{\text{target}, i}^2\label{eq-finalstep},
\end{align}
where Eqn~(\ref{eq-step1}) is derived from the fact that all the elements of $\boldsymbol{x}_{\text{target}}$ are normalized into $(0,1)$.
Further, by substituting Eqn~(\ref{eq-l2norm}) into Eqn~(\ref{eq-step1}), we obtain Eqn~(\ref{eq-finalstep}), which is an upper bound for  $\text{MSE}(\hat{\boldsymbol{x}}_{\text{target}}, \boldsymbol{x}_{\text{target}})$.
% which is $\frac{1}{d_{\text{target}}}\sum^{d_{\text{target}}}_{i=1} 2x_{\text{target}, i}^2$.
%

\begin{table*}[t]
\caption{Results of ablation study based on LR with Bank marketing}
\centering
\begin{tabular}{c c c c c c}
\toprule
Case Index & Input $\boldsymbol{x}_{\text{adv}}$ & Input Noise & Constraint on $\hat{\boldsymbol{x}}_{\text{target}}$ & Generator & MSE \\
\toprule
1&	$\times$&	$\surd$&	$\surd$&	$\surd$&	0.1705  \\
2&	$\surd$&	$\times$&	$\surd$&	$\surd$&	0.1514\\
3&	$\surd$&	$\surd$&	$\times$&	$\surd$&	0.1474\\
4&	$\surd$&	$\surd$&	$\surd$&	$\times$&	0.2862\\
5&	$\surd$&	$\surd$&	$\surd$&	$\surd$&	0.1216\\
6 &	$\times$&	$\times$&	$\times$&	$\times$&	0.2459\\
\bottomrule
\end{tabular}
\label{tab-ablation}
\end{table*}


Upon that, we compute the upper bound for Bank, Credit, Drive and News datasets, which are 0.60, 0.14, 0.45 and 0.34, respectively. In general, the larger the upper bound is, the worse the attack accuracy the adversary could achieve. This explains why the MSE of Bank increases faster than others.
%These upper bounds are consistent with the results shown in Fig.~\ref{fig:esa-performance}, and can also explain why the increase of the MSE on Bank is much larger than that on other datasets, since the MSE bound on Bank is largest.
Besides, ESA achieves better results on Drive than on News as the adversary has more equations (i.e., $c-1 = 10$) for Drive than those for News (i.e., $c-1 = 4$). %, which contains more information.

%as the coefficient matrix $\boldsymbol{\Theta}^{(\text{Drive})}_{\text{target}}$ with dimension $10\times d_{\text{target}}$ contains more information about $\boldsymbol{x}_{\text{target}}$ than $\boldsymbol{\Theta}^{(\text{News})}_{\text{target}}$ with dimension $4\times d_{\text{target}}$.

% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }



\vspace{1mm}\noindent
\textbf{Effect of $d_{\text{target}}$ on PRA.} Fig.~\ref{fig:pra-performance} shows the attack performance of PRA \textit{w.r.t.} CBR. %The attack accuracy on the drive diagnosis dataset in Fig.~\ref{subfig:pra-drive} is higher than on other datasets. This is because there are 11 classes in this dataset, thus given the predicted class, the adversary can eliminate more prediction paths, resulting in a better performance.
Notice that the comparison between PRA and the random guess methods is similar to Fig.~\ref{fig:esa-performance}, where the attack accuracy degrades as the fraction of $d_{\text{target}}$ goes up. In general, more target features would lead to more possible prediction paths. Therefore, the probability for the adversary to select the correct path is reduced.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

Note that the CBR of Drive is stable or even slightly increases as $d_{\text{target}}$ increases. There are two reasons.
%
First, the Drive dataset has 11 classes, which is much more than those in the other datasets (2 in Bank and Credit, 5 in News).
%
As such, in Drive, each class corresponds to a smaller number of tree paths.
%
Therefore, given one specific class, there exist only a small number of candidate prediction paths, which leads an improved CBR.
%
In this case, the adversary would not gain a significant advantage by knowing more features.
%The possible prediction paths of one specific class can be therefore greatly reduced, leading to a sufficiently good CBR. And more known features may not facilitate further restrictions.
%
Second, the decision tree model only selects informative features during training, which means the increase of $d_{\text{target}}$ in Drive does not necessarily increase the number of unknown features in the tree, since some features may never be selected. As a consequence, a larger $d_{\text{target}}$ do not always decrease the CBR of the PRA attack.

%On the one hand, the possible prediction paths are greatly restricted given the predicted class, thus, more known features cannot facilitate further restrictions. On the other hand, since decision tree only selects a subset of features during model building and the tree depth is 5 in our experiments, even the fraction $d_{\text{target}}$ increases, the number of target features in the model does not necessarily increase due to the randomness.

% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }


%\noindent\textbf{Variables.} (1) the percentage of unknown features, e.g., 10\%, 30\%, 50\%, 70\%, 90\%. (2) datasets. (3) binary LR, multi-class LR, and DT. (4) equality solving attack and path restriction attack.



\begin{figure*}[t]
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-bank-grn-cbr.pdf}
  %\vspace{-2mm}
  \caption{Bank marketing}
  \label{subfig:grna-bank-rf-cbr}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-credit-grn-cbr.pdf}
  %\vspace{-2mm}
  \caption{Credit card}
  \label{subfig:grna-credit-rf-cbr}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-drive-grn-cbr.pdf}
  %\vspace{-2mm}
  \caption{Drive diagnosis}
  \label{subfig:grna-drive-rf-cbr}
\end{subfigure}
~
\begin{subfigure}[b]{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-news-grn-cbr.pdf}
  %\vspace{-2mm}
  \caption{News popularity}
  \label{subfig:grna-news-rf-cbr}
\end{subfigure}

\caption{Evaluation of generative regression network attack on the RF model \textit{w.r.t.} CBR}
% \vspace{-0.5cm}
\label{fig:grna-rf-performance-cbr}
%\vspace{2mm}
\end{figure*}

\begin{figure*}[t]
\begin{subfigure}[b]{.48\columnwidth}
  \centering
  % include first image
  \includegraphics[width=0.95\columnwidth]{figures/fig-sample-size-syn1-135.pdf}
  %\vspace{-2mm}
  \caption{Synthetic dataset 1}
  \label{subfig:synthetic-1}
\end{subfigure}
~
\begin{subfigure}[b]{.48\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-sample-size-syn2-135.pdf}
  %\vspace{-2mm}
  \caption{Synthetic dataset 2}
  \label{subfig:synthetic-2}
\end{subfigure}
~
\begin{subfigure}[b]{.48\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-sample-size-drive-135.pdf}
  %\vspace{-2mm}
  \caption{Drive diagnosis}
  \label{subfig:drive-size}
\end{subfigure}
~
\begin{subfigure}[b]{.48\columnwidth}
  \centering
  % include second image
  \includegraphics[width=0.95\columnwidth]{figures/fig-sample-size-news-135.pdf}
  %\vspace{-2mm}
  \caption{News popularity}
  \label{subfig:news-size}
\end{subfigure}
\caption{Effect of number of predictions \textit{w.r.t.} MSE per feature}
% \vspace{-0.2cm}
\label{fig:grn-sample-size}
%\vspace{2mm}
\end{figure*}



\subsection{Evaluation of Attacks Based on Multiple Predictions}
\label{subsec:experiments:multiple}

%\noindent\textbf{Variables.} (1) the percentage of unknown features, e.g., 10\%, 20\%, 30\%, 40\%, 50\% 60\%. (2) datasets. (3) generator attack (LR, NN, RF). (4) fraction of samples used in the general attack, e.g., 20\%, 40\%, 60\%, 80\%, 100\% of the prediction dataset. \textit{If needed: (5) Background information level: known mean, known distribution, etc. (how to introduce the reason of using these information.)}


The generator model of GRNA is a multilayer perceptron with an input layer with size $d$, an output layer with size $d_{\text{target}}$, and three hidden layers (with 600, 200, 100 neurons, respectively). Besides, we employ Layer Normalization~\cite{ba2016layer} after each hidden layer to stabilize the hidden states. For the model that imitates the RF model (see Section~\ref{subsec:attack-rf}), inspired by~\cite{biau2019neural}, we apply another multilayer perceptron with two hidden layers (with 2000 and 200 neurons, respectively).

\vspace{1mm}\noindent
\textbf{Ablation Study on GRNA.}
We first conduct ablation studies on GRN to test the impacts of its different components on the attack performance. The training dataset is Bank marketing, target model is LR, and $40\%$ features of Bank is randomly selected as the $\boldsymbol{x}_{\text{target}}$. We show the experimental results in Table~\ref{tab-ablation}.
In general, we test the following branches: the inputs of the generator are exclusively noises (case 1); the input of the generator is exclusively $\boldsymbol{x}_{\text{adv}}$ (case 2); no converge constraints are added to the generator output $\hat{\boldsymbol{x}}_{\text{target}}$ (case 3); the generator is removed, i.e., a naive regression model which infers $\boldsymbol{x}_{\text{target}}$ based solely on the federated model $f$ and the model output $v$  (case 4). In addition, we show the results of the original GRN (case 5) and random guess (case 6) for comparison.

From Table~\ref{tab-ablation}, we observe that the naive regression model performs worse than random guess (case 4). The reason is that without constraints of $\boldsymbol{x}_{\text{adv}}$, the inferred values of $\hat{\boldsymbol{x}}_{\text{target}}$ regressed from the federated model tend to diverge. We also see that the performance of the generator without $\boldsymbol{x}_{\text{adv}}$ as input degrades most (case 1), which is expected since the effectiveness of GRN mainly relies on the correlations between $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{x}_{\text{target}}$. As mentioned in Section~\ref{subsec:attacks-grn}, we penalize the variance of  $\hat{\boldsymbol{x}}_{\text{target}}$ when it it too large to prevent GRN from generating meaningless samples. Case 3 shows that the constraint on $\hat{\boldsymbol{x}}_{\text{target}}$ can reduce the inference error by $17\%$.
In addition, we observe that the random vector, which is concatenated with $\boldsymbol{x}_{\text{adv}}$ as the input of GRN, can further reduce the reconstruction error by $20\%$ (case 2).

\vspace{1mm}\noindent
\textbf{Effect of $d_{\text{target}}$ on GRNA.}
Fig.~\ref{fig:grna-performance} shows the attack performance of GRNA for three models (i.e., LR, RF, and NN) on four real-world datasets \textit{w.r.t.} MSE per feature. Similarly, we vary the fraction of $d_{\text{target}}$.
%
The trends of the three models on all the datasets are similar, i.e., the MSE per feature all goes up as the fraction of $d_{\text{target}}$ increases. This is because GRNA relies on the feature correlations between $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{x}_{\text{target}}$ to infer the unknown feature values. The learned correlations would become weaker if the fraction of $d_{\text{target}}$ is larger, leading to relatively worse attack performance. However, even when the fraction of $d_{\text{target}}$ is 60\%, the GRNA still achieves a much better inference than the random guess methods, demonstrating its effectiveness.
%We have three main observations.
%First, all the values inferred by GRN are closer to the ground truth of $x_{target}$ than values guessed randomly, which is expected because GRN could accurately recreate $x_{target}$ by learning the distribution of $D_{target}$.
In addition, GRNA with the NN model performs better than that with the LR and RF models. The reason is that the NN model has more complicated decision boundaries than the other two models, thus greatly limiting the possible distributions of ${\boldsymbol{x}}_{\text{target}}$ given the same $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{v}$. Meanwhile, with more parameters, the NN model itself can capture more important information about the feature correlations than others, resulting in better attack performance.
%GRN achieves better performance with mean constraints than the performance without mean information. However, even without any auxiliary information, GRN could recreate $x_{target}$ with a far less error than random guess, which demonstrates the inference effectiveness of the proposed framework.

As the NN model imitating the RF model only approximates the feature thresholds on the internal tree nodes, we also apply the CBR metric for evaluating GRNA on the RF model. Fig.~\ref{fig:grna-rf-performance-cbr} illustrates the performance for varying the fraction of $d_{\text{target}}$.
%
Results demonstrate that GRNA recovers many more branches in the trees than the random guess methods. For example, if the fraction of $d_{\text{target}}$ is 10\%, GRNA correctly infers more than 80\% of the tree branches \textit{w.r.t.} the bank marketing and drive diagnosis datasets given the generated feature values.




\vspace{1mm}\noindent
\textbf{Effect of $n$ in the prediction dataset on GRNA.} As the generator model is trained on multiple predictions,
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }
we investigate the effect of the number of predictions $n$ using two synthetic datasets and two real-world datasets.
%
For a dataset $\mathcal{D}$, we first use half of the dataset for model training and testing, then randomly select $n = \{10\%, 30\%, 50\%\}\times |\mathcal{D}|$ samples from the remaining part as the prediction dataset to train the generator using GRNA.
%
Fig.~\ref{fig:grn-sample-size} shows the attack performance \textit{w.r.t.} MSE per feature. Overall speaking, the trends on the four datasets demonstrate that the more samples in the prediction dataset, the less MSE per feature the adversary can obtain.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }
In other words, the adversary could accumulate more prediction outputs in the long term to improve his attack accuracy.

\begin{figure*}
\centering
    \begin{subfigure}[b]{0.4\textwidth}
            \includegraphics[width=\columnwidth]{figures/bank-rf-corr.pdf}
            \caption{Bank marketing (LR model)}
            \label{fig-bank-corr}
    \end{subfigure}%
    \hspace{2mm}
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/credit-lr-corr.pdf}
            \caption{Credit card (RF model)}
            \label{fig-credit-corr}
    \end{subfigure}
    \caption{Effect of data correlations between each feature in $\boldsymbol{x}_{\text{target}}$ with $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{v}$}
    \label{fig-corre}
\end{figure*}

\begin{figure*}
\centering
    \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\columnwidth]{figures/fig-round-bank-esa.pdf}
            \caption{ESA on bank marketing}
            \label{subfig:bank-conf-esa}
    \end{subfigure}%
    ~
    \hspace{2mm}
    \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/fig-round-drive-esa.pdf}
            \caption{ESA on drive diagnosis}
            \label{subfig:drive-conf-esa}
    \end{subfigure}
    ~
    \hspace{2mm}
    \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\columnwidth]{figures/fig-round-bank-grn.pdf}
            \caption{GRNA on bank marketing}
            \label{subfig:bank-conf-grn}
    \end{subfigure}%

\vspace{2mm}
\centering
    \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\columnwidth]{figures/fig-round-drive-grn.pdf}
            \caption{GRNA on drive diagnosis}
            \label{subfig:drive-conf-grn}
    \end{subfigure}%
    ~
    \hspace{2mm}
    \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\columnwidth]{figures/fig-dropout-credit-grn.pdf}
            \caption{GRNA on credit card}
            \label{subfig:credit-dropout-grn}
    \end{subfigure}%
    ~
    \hspace{2mm}
    \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/fig-dropout-credit-grn.pdf}
            \caption{GRNA on news popularity}
            \label{subfig:news-dropout-grn}
    \end{subfigure}
    \caption{Evaluation of countermeasures: (a)-(b) and (c)-(d) illustrate the effects of the rounding strategy in ESA and GRNA \textit{w.r.t.} the LR model, respectively; (e)-(f) illustrate the effect of the dropout strategy in GRNA \textit{w.r.t.} the NN model.}
    \label{fig-countermeasures}
    \vspace{-0.5cm}
\end{figure*}

\vspace{1mm}\noindent
\textbf{Effect of data correlations on GRNA.}
Notice that the performances of the LR and RF models are lower than that of the NN model (see Fig.~\ref{fig:grna-performance}).
The reason is that a small part of the inferred feature values is far from the ground-truth, leading to a relatively low overall attack performance.
To further explore this phenomenon, we analyze the impact of data correlations between each target feature in $\boldsymbol{x}_{\text{target}}$ and the adversary's features $\boldsymbol{x}_{\text{adv}}$ as well as the prediction output $\boldsymbol{v}$.
%
%We utilize the average Pearson correlation coefficient between each feature in $\boldsymbol{x}_{\text{target}}$ with $\boldsymbol{x}_{\text{adv}}$ and $\hat{\boldsymbol{v}}$, respectively.
Specifically, the data correlation is defined as
\begin{align}
% \nonumber % Remove numbering (before each equation)
  \label{eq-adv}
  \textit{corr}(\boldsymbol{x}_{\text{adv}}, \boldsymbol{x}_{\text{target}, i}) & = \frac{1}{d_{\text{adv}}} \sum\limits^{d_{\text{adv}}}_{j=1} abs(r(\boldsymbol{x}_{\text{adv}, j}, \boldsymbol{x}_{\text{target}, i})), \\
   \label{eq-yhat}
   \textit{corr}(\boldsymbol{v}, \boldsymbol{x}_{\text{target}, i}) & = \frac{1}{c}\sum\limits^{c}_{j=1} abs(r(v_j, \boldsymbol{x}_{\text{target}, i})),
\end{align}
where $r(a,b)$ denotes the Pearson correlation coefficient between $a$ and $b$, and $abs(\cdot)$ denotes the absolute coefficient. The absolute value is adopted to focus on the magnitude of correlations. Essentially, the larger the two coefficients are, the easier the adversary can learn the feature correlations via GRNA.

Fig.~\ref{fig-corre} shows the correlations computed by Eqn~(\ref{eq-adv}) and~(\ref{eq-yhat}). The fractions of $d_{\text{target}}$ used for the bank marketing (in Fig.~\ref{fig-bank-corr}) and credit card (in Fig.~\ref{fig-credit-corr}) datasets are 40\% and 30\%, respectively. In addition, the x-axis represents the MSE for each feature in $\boldsymbol{x}_{\text{target}}$.
%
We can observe that the correlations \textit{w.r.t.} both $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{v}$ impact the attack performance of GRNA.
%
A weaker correlation between $\boldsymbol{x}_{\text{target}, i}$ with $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{v}$ results in a lower inference accuracy, such as features 1 and 3 in Fig.~\ref{fig-bank-corr} and features 4 and 6 in Fig.~\ref{fig-credit-corr}.
%
The rationale is that a weak correlation implies that the change of the unknown feature value only has a minor impact on the generated sample and the prediction output; thus, its value range is broader than the other unknown features, leading to an inaccurate inference.
%
%These results provide useful insight for designing vertical FL algorithms: reducing those closely related features owned by different parties can enhance privacy protection against the proposed feature inference attack.

% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }

Another insight is that GRNA can achieve different reconstruction accuracy regarding different features. The MSE metric computed by Eqn~(\ref{eq:mse-per-feature}), which averages the reconstruction errors on all target features, is mainly used to evaluate the overall performance of our attacks. In real-world applications, we should note that features closely correlated to $\boldsymbol{x}_{\text{adv}}$ can be more precisely reconstructed than the relatively independent ones. For example, after obtaining the inferred deposit and shopping information based on a user's income, the adversary may be more convinced of the inferred deposit as it is more relevant to the income feature.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }

%%%\subsection{Summary}\label{subsec:summary}
%For all the proposed attacks, ESA, PRA, and GRNA, the attack performance is much better than the baselines.
%%%The attack performance of all the proposed attacks is much better than the baselines.
%Given individual prediction output, our attacks, ESA and PRA, are much better than the random guess method.
%%%In particular, ESA can precisely recover $P_{\text{target}}$'s feature values if $c > d_{\text{target}}$, and PRA can correctly infer most branches in the tree model.
%when $c > d_{\text{target}}$, ESA precisely recovers the attack target's feature values.
%%%Meanwhile, the attack performance of GRNA could be improved if $P_{\text{adv}}$ accumulates many prediction outputs or $P_{\text{adv}}$'s features are highly correlated with the attack target's features.
%Given multiple prediction outputs, the general attack GRNA we proposed is well applicable to three types of vertical FL models and also has a higher attack accuracy than the random guess method.
%%%These observations provide several useful insights on protecting model predictions in vertical FL collaboration:
%%%(i) the passive parties should carefully check the relationship between the number of classes and the number of their contributed features, ensuring no obvious privacy vulnerabilities;
%%%(ii) the parties should jointly execute a secure algorithm to compute their feature correlations and remove those closely related features before starting the vertical FL training and prediction;
%%%(iii) the passive parties should be vigilant if the active party has requested a lot of predictions using the same trained model, as from which the active party may initiate a more powerful attack.



\begin{comment}
\begin{figure*}
\centering
    \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=\columnwidth]{figures/syn-5005-predict.pdf}
            \caption{Synthetic Dataset (50 features)}
            \label{fig-predict-incr-5005}
    \end{subfigure}%
    \hspace{2mm}
    \begin{subfigure}[b]{0.48\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/syn-2510-predict.pdf}
            \caption{Synthetic Dataset (25 features)}
            \label{fig-predict-incr-2510}
    \end{subfigure}
    \caption{Attack effects to NN with various prediction samples.}\label{fig-dropout}
\end{figure*}
\end{comment} 

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-introduction.tex <==
\section{Introduction}\label{sec:introduction}

Recent years have witnessed a growing interest in exploiting data from distributed sources of multiple organizations, for designing sophisticated machine learning (ML) models and providing better customer service and acquisition. 
%
However, proprietary data cannot be directly shared for two reasons.
%
On the one hand, the usage of user’s sensitive data is compelled to abide by standard privacy regulations or laws, e.g., GDPR \cite{GDPR2016} or CCPA \cite{CCPA2018}. 
%
On the other hand, the data is a valuable asset to the organizations for maintaining a competitive advantage in business, which should be highly protected.

Federated learning (FL) \cite{WuCXCO20, Bonawitz17, McMahanMRHA17, Zheng2019, choudhury2020anonymizing, YangLCT19} is an emerging paradigm for data collaboration that enables multiple data owners (i.e., parties) to jointly build an ML model and serve new requests without revealing their private data to each other. 
%
%There are two typical FL scenarios: horizontal FL (HFL) and vertical FL (VFL). In HFL, the parties have the same features but share no sample; while in VFL, all parties have the same set of samples, but each party only has a disjoint subset of features and only one party holds the label \cite{YangLCT19}. 
%
FL can be categorized into different scenarios according to the data partitioning. In this paper, we consider vertical FL \cite{HuNYZ19, VaidyaCKP08, ChengCorr19, OhrimenkoSFMNVC16, WuCXCO20, HeYCGH20} where the participating parties hold the same set of samples while each party only has a disjoint subset of features.
%
Vertical FL has been demonstrated effective in many real-world applications and received increased attention in organizations or companies \cite{ChengCorr19, OhrimenkoSFMNVC16}. 
%Meanwhile, only one party owns the label information, which called \textit{active party}. The other parties are called \textit{passive parties}.
%
Fig.~\ref{fig:vertical-fl-example} illustrates a digital banking example. A bank aims to build an ML model to evaluate whether to approve a user's credit card application by incorporating more features from a Fintech company. 
%
The bank holds features of `age' and `income' while the Fintech company holds features of `deposit' and `average online shopping times'. Only the bank owns the label information in the \textit{training dataset} and \textit{testing dataset}, i.e., the ground truth that indicates whether an application should be approved. We refer to the party with the label as the \textit{active party} and the other parties as \textit{passive parties}.
%
To train a vertical FL model, the parties iteratively exchange certain intermediate results in a secure manner until obtaining a jointly trained model \cite{WuCXCO20}.
%
Finally, the trained model will be released to the parties for justifying the model's effectiveness and interpretability. 


%The basic idea of FL training is to iteratively let each party (i) perform some local computations on her data to derive certain intermediate results, and then (ii) exchange these results with other parties in a secure manner to advance the training process, until a final model is obtained \cite{WuCXCO20}.
%
After obtaining the trained model, the parties utilize it to collaboratively compute model predictions for new samples in the \textit{prediction dataset}, for example, new credit card applicants in Fig.~\ref{fig:vertical-fl-example}. 
%As the features of new sample are distributed among all parties, the parties need to compute the predictions collaboratively. 
In practice, the prediction outputs will be revealed to the active party for making further decisions. 
%
Though cryptographic techniques, e.g., partially homomorphic encryption \cite{Paillier99, Damg01, WuWZLCL18} and secure multiparty computation \cite{Yao82b, DamgardPSZ12}, can be applied to ensure that no intermediate information during the computation is disclosed \cite{WuCXCO20}, the prediction outputs must contain information of the parties' sensitive data because they are computed upon the private data. 
%
Therefore, in this paper, we aim to investigate the key question: \textit{how much information about a passive party's feature values can be inferred by the active party from the model predictions in vertical FL?}

%Given the trained FL model, the parties can make model predictions for new samples. While every party can execute predictions at local in HFL as each has all features, the parties need to collaborate with each other for the computation in VFL since the features of a sample are distributed among them. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/v-splitting.pdf}
    \caption{Example of vertical federated learning}
    \label{fig:vertical-fl-example}
    \vspace{-5mm}
\end{figure}

Although a number of feature inference attacks are proposed against machine learning~\cite{NasrSH2019, Carlini18, MelisSCS19, hitaj2017deep, ZhuLH19, wang2019beyond, fredrikson2014privacy, fredrikson2015model, yeom2018privacy}, none of them are applicable to our problem. 
%%% ooibc: none takes plural form although "is" is correct too, but "are" is more commonly used
%
%
Many existing attacks \cite{NasrSH2019, MelisSCS19, ZhuLH19, hitaj2017deep, wang2019beyond, Carlini18} aim to infer a participating party's feature values in the horizontal FL scenario \cite{Bonawitz17, McMahanMRHA17, Zheng2019, choudhury2020anonymizing}, where the parties have the same features but with different samples. 
%
However, these attacks greatly rely on the model gradients 
%%% ooibc: sounds awkward
%% iterated exchange of model gradients?
%%% wyc: revised to "rely on the model gradients exchanged"
exchanged during the training process, which unintentionally memorize sensitive information of the training samples.
%
Once the model gradients are safely protected, e.g., using cryptographic techniques \cite{Bonawitz17, Zheng2019}, these attacks would be invalid. 
%%% ooibc: last half is cryptic 
%
Also, for the inference attack in the prediction stage (i.e., considered in this paper), 
the FL model 
%%never saw 
is not aware of the predicting samples beforehand. 
Thus, the memorization nature used in these attacks does not work. 
%
Another thread of feature inference attacks~\cite{fredrikson2014privacy, fredrikson2015model, yeom2018privacy} assumes that the adversary could obtain some auxiliary statistics or marginal data distribution about the unknown features. 
%
This assumption is relatively strong, as it is challenging in practice for the active party to collect such background information from the passive parties in vertical FL. 
%%A more detailed discussion of related work is presented in Section~\ref{sec:related-work}.
%%% ooibc: the sentence does not help but break the flow
%%% instead, a sentence of summary that helps to motivate the work would be better -- it helps to connect to the next para
%There exist a number of inference attacks \cite{Salem0HBF019, ShokriSSS17, NasrSH2019, MelisSCS19, hitaj2017deep, ZhuLH19, wang2019beyond} in horizontal FL \cite{Bonawitz17, McMahanMRHA17, McMahanRT018, Zheng2019, BhagojiCMC19, NikolaenkoWIJBT13, choudhury2020anonymizing, YangLCT19}, which assumes that the parties have the same features but with different samples. 
%However, to our knowledge, no work explores the privacy leakages in vertical FL. Meanwhile, none of the existing attack methods are applicable to our problem. 
%
%First, the membership inference attack \cite{Salem0HBF019, ShokriSSS17, NasrSH2019}, which tries to determine whether a particular record is in the training data or not, does not exist in vertical FL because intrinsically, every party knows all the training sample ids. 
%
%Second, require full training data. 
%
%Second, another line of attack methods \cite{MelisSCS19, ZhuLH19, hitaj2017deep, wang2019beyond} aim to infer interesting properties or revert feature values of other parties, relying on the iterative model gradients in the training stage of horizontal FL. However, these methods are only specific to certain horizontal FL algorithms.
%
%Third, several feature inference attack methods~\cite{fredrikson2014privacy, fredrikson2015model, yeom2018privacy} assume that the adversary can obtain some background information (e.g., statistics or marginal data distribution) about the unknown features. This assumption is rather strong in vertical FL, as it is often challenging in practice for the active party to collect such background information from the passive parties. 
%Though FL provides reasonable privacy protections on the parties' sensitive data, recent studies have demonstrated that existing FL algorithms are vulnerable to various attacks, including membership inference attack, property inference attack, feature inference attack. A challenge to infer features in prediction phase is that the trained model never saw prediction samples before, thus we can not rely on the memorization nature~\cite{nasr2019comprehensive, carlini2018secret}, i.e., models could unintentionally memorize training inputs, or overfitting nature~\cite{shokri2017membership, salem2018ml} of ML algorithms.
%To investigate 
%%% ooibc: explore?
%%% prevent / investigate?
%%% wyc: revised to investigate
%%% ooibc: the whole sentence does not sound right
%the privacy leakages in the prediction stage of vertical FL for providing insights on how to design the corresponding privacy-preserving algorithms, we present several feature inference attacks based on model predictions.


%%% ooibc:
%% In this paper, we study the privacy leakage problem in the prediction of vertical FL, and present ...? (nothing is said about privacy preserving elsewhere)
%%% wyc: yes, I comment out the previous sentence
In this paper, we study the privacy leakage problem in the prediction stage of vertical FL, by presenting several feature inference attacks based on model predictions. 
%
%These potential privacy leakages are considered when designing privacy-preserving vertical FL algorithms in our \textit{Falcon}\footnote{\url{https://www.comp.nus.edu.sg/~dbsystem/fintech-Falcon/}} system.
%
Our attack methods do not rely on any intermediate information during the computation of prediction outputs. For example, we assume that the parties can jointly run a secure protocol such that only the prediction outputs are released to the active party and nothing else. 
%
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }
Besides, unlike previous work \cite{fredrikson2014privacy, fredrikson2015model, zhang2020secret}, the proposed methods need no statistics or distributions of the attack target's data.
Therefore, we consider the most stringent setting that the active party (i.e., the adversary) controls only the trained vertical FL model and the model predictions.  
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }

%Besides, no background information (e.g., the statistics of the passive parties' features) is required for the attacks. 
%
%Therefore, we consider the most stringent setting that the active party (i.e., the adversary) controls only the trained vertical FL model and the model predictions. 
%\textit{(add discussion about insights as well as defense methods and back to our Falcon system).}
From the experimental results, we observe that those model predictions can leak considerable information about the features held by the passive parties, especially when specific conditions are satisfied, e.g., the number of classes in the classification is large or the adversary's features and the passive parties' features are highly correlated. 
%
In light of these observations, we design several defense strategies and incorporate them into our \textit{Falcon}\footnote{\label{note:falcon}\url{https://www.comp.nus.edu.sg/~dbsystem/fintech-Falcon/}} (federated learning with privacy protection) system to safeguard against such potential privacy risks.

Specifically, we make the following contributions.
\begin{itemize}[topsep=2pt,itemsep=2pt,parsep=0pt,partopsep=0pt,leftmargin=15pt]
    \item We formulate the problem of feature inference attack on model predictions in vertical FL, where the active party attempts to infer the feature values of new samples belong to the passive parties. To the best of our knowledge, this is the first work that investigates this form of privacy leakage in vertical FL.
    \item We propose two specific attacks on the logistic regression (LR) and decision tree (DT) models when the adversary only has an individual prediction output. These attacks are straightforward to initiate and can achieve high accuracy when certain conditions are satisfied.
    \item We further design a general inference attack which can learn the correlations between the adversary's features and the attack target's features based on multiple predictions accumulated by the adversary. This attack can handle more complex models, such as neural networks (NN) and random forest (RF). %Essentially, this attack method learns the feature correlation between the adversary and the attack target is based on generative matching networks (GMNs) and can be applied to any vertical FL model.
    \item We implement the proposed attacks and conduct extensive evaluations on both real-world and synthetic datasets. 
    The results demonstrate the effectiveness of our attacks and highlight the need for designing defense mechanisms to mitigate the privacy risks arising from federated model predictions. 
    We also analyze and suggest several potential countermeasures against these attacks.
    %%% ooibc: the last sentence is neither here nor there s
\end{itemize}





\begin{comment}
Traditional machine learning (ML) algorithms need to gather and store data in a centralized server before training, which incurs considerable concerns over transmitting private information~\cite{li2020federated}. To mitigate such privacy risks, federated learning (FL) was first proposed in~\cite{mcmahan2017communication}. In FL, each client trains a local model on the dataset owned by themselves, then aggregates model gradients or intermediate outputs into a global model, eliminating the privacy risk of transmitting data. FL could be further categorized into horizontal FL and vertical FL, in which datasets spread among clients by records or features respectively~\cite{YangLCT19}. Fig.~\ref{fig-intro} shows two examples of horizontal splitting and vertical splitting respectively. With mitigating privacy concerns and data isolations, horizontal FL is now widely applied among edge devices~\cite{YangLCT19, li2020federated}, while vertical FL starts receiving increased attention among companies and organizations~\cite{YangLCT19, WuCXCO20}.

\begin{figure}
\centering
    \begin{subfigure}[b]{0.5\textwidth}
            \includegraphics[width=\columnwidth]{figures/h-splitting.pdf}
            \caption{Horizontal Splitting.}
    \end{subfigure}%
    \hspace{5mm}
    \begin{subfigure}[b]{0.5\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/v-splitting.pdf}
            \caption{Vertical Splitting.}
    \end{subfigure}
    \caption{Examples of horizontal and vertical splitting.}\label{fig-intro}
\end{figure}

Some most recent studies, however, have demonstrated that FL is vulnerable to membership inference~\cite{nasr2019comprehensive}, property inference~\cite{MelisSCS19} and feature inference~\cite{hitaj2017deep, wang2019beyond} (or model inversion in some literature). Membership inference~\cite{nasr2019comprehensive} aims to determine whether a record is in the training set or not, while property inference~\cite{MelisSCS19} aims to learn global statistics of training set.
Though performing different inference tasks, the core ideas of~\cite{nasr2019comprehensive} and~\cite{MelisSCS19} are similar, i.e., training attacking models on global shared gradients or network parameters. Further, \textit{feature inference}~\cite{hitaj2017deep, wang2019beyond} seeks to accurately recreate features that are used in the training dataset.
For example, \cite{hitaj2017deep} and \cite{wang2019beyond} employ generative
adversarial network (GAN) to recover training pictures from other clients. While demonstrating good results, the effectiveness of these attacks is limited by the discriminator of GAN, i.e. the global trained model in FL. In this paper, we focus on feature inference attack.

Generally, global shared model parameters or gradients are indispensable to most recent attacks. In horizontal FL~\cite{mcmahan2017communication, choudhury2020anonymizing, YangLCT19, li2020federated}, each client agrees on a pre-defined model structure and shares gradient updates periodically. While in vertical FL~\cite{hardy2017private, liu2018secure, cheng2019secureboost, hu2019fdml, WuCXCO20}, only limited intermediate model outputs are shared during training, which means current attacks~\cite{NasrSH2019, MelisSCS19, hitaj2017deep, wang2019beyond} are only applicable to horizontal FL, instead of vertical FL.

There are two main challenges when designing attacks to vertical FL: first, the local model parameters and gradients trained by each client are strictly private to each other during training and testing phase~\cite{hardy2017private, liu2018secure, cheng2019secureboost, hu2019fdml, WuCXCO20}, which means traditional white-box attacking methods targeting training phase could not be adapted to this case; second, traditional feature inference methods~\cite{fredrikson2014privacy, fredrikson2015model, yeom2018privacy, zhu2019deep, hitaj2017deep, wang2019beyond} need feature priors or other auxiliary information to enhance the accuracy of inference results. While in vertical FL, clients' data is strictly private to each other~\cite{WuCXCO20}, making it difficult for attackers to attain such auxiliary information.

In this paper, we propose a general attack framework to infer features in the prediction phase of vertical FL. Most vertical FL studies~\cite{hardy2017private, liu2018secure, cheng2019secureboost, hu2019fdml} focus on designing privacy-preserving schemes to protect input data during training and testing phase, while few of them notice the security issue in prediction phase.
Generally, in vertical FL, clients need to aggregate local models and publish the aggregated model to each other after training for model quality and explanation assessment~\cite{WuCXCO20}.
We demonstrate that private information in prediction dataset could be inferred from this trained model.
A challenge to infer features in prediction phase is that the trained model never saw prediction samples before, thus we can not rely on the memorization nature~\cite{nasr2019comprehensive, carlini2018secret}, i.e., models could unintentionally memorize training inputs, or overfitting nature~\cite{shokri2017membership, salem2018ml} of ML algorithms.

The structure of this paper is as follows.
\begin{enumerate}
    \item \textbf{Introduction}. (1) FL introduction, vertical FL. (2) Attacks on horizontal FL. (3) vulnerabilities in the vertical FL prediction stage. (4) Our contributions.
    \item \textbf{Background}. (1) machine learning. (2) FL and vertical FL. 
    \item \textbf{Problem statement}. (1) system model. (2) threat model. (3) vertical FL prediction. (4) attack metrics.
    \item \textbf{Attacks on LR and NN}. (1) specific condition attack. (2) generative regression networks attack.
    \item \textbf{Attacks on tree-based models}. (1) single tree attack. (2) ensemble model attack. 
    \item \textbf{Experimental evaluations}. (1) setup: dataset, models, metric. (2) attacks on LR and NN. (3) attacks on tree-based models. (4) summary.
    \item \textbf{Countermeasures}. (1) rounding confidence score. (2) dropout for NN. (3) post-verification. (4) not reveal model, instead of using interpretability scores. 
    \item \textbf{Related work}. (1) FL and vertical FL. (2) horizontal FL attacks.
    \item \textbf{Conclusions}.
\end{enumerate}

To address such problem, we propose to learn correlations between attacker's feature set $x_{adv}$ and targeting feature set  $x_{target}$ via a generative network in an unsupervised manner.
We argue that correlations exist between $x_{adv}$ and $x_{target}$, or the models trained by vertical FL could not perform better than the local models trained respectively on $x_{adv}$ and $x_{target}$.
The experimental results demonstrate that our attacking framework could effectively recreate target features even without auxiliary information like feature priors. To summarize, we make the following observations:
\begin{enumerate}
    \item Existing works mainly focus on attacks in the horizontal federated learning (HFL) scenario, no work considers the privacy leakages in vertical federated learning (VFL) scenario.
    \item Privacy leakages in the prediction stage is an important aspect, because there could be a large number of predictions in the production system.
    \item Unlike the attacks in HFL, there is no black-box attack in VFL. An attacker does not have the features of the target party, therefore, he cannot query the model prediction API with unlimited samples (i.e., a fundamental assumption in black-box attacks in HFL).
\end{enumerate}
\end{comment}

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-poisoning-attacks.tex <==
\section{Poisoning Attacks}\label{sec:poisoning-attacks}

In this section, we present two kinds of data poisoning attacks: \textbf{random noise attack} and \textbf{correlated pattern attack}. The goal of the attacks is to decrease the model accuracy. Both attacks are initiated by the ordinary clients. The former attack is achieved by providing useless features with random noise, while the latter attack is achieved by providing features that are highly correlated to labels to backdoor the trained model. \par 

\subsection{Random Noise Attack}\label{subsec:random-noise-attack}

This attack injects some random noises to the local training dataset, to decrease the accuracy of the trained model. \textit{(Naive)}.

\subsection{Correlated Pattern Attack}\label{subsec:correlated-pattern-attack}

This attack assumes that the attacker has some background knowledge, i.e., a small subset (e.g., 5\%) of labels of samples in the training dataset. This assumption is reasonable in the malicious setting, for example, a business competitor of the super client may collude with an ordinary client and provide the labels of some overlapped samples in the training dataset. \par

Given the small subset of labeled samples, the attacker can train a classifier using its local features, and predict the labels of the rest of samples in the training dataset. After obtaining these labels, the attacker may modify the values of its local features to correlate to the labels, resulting in a backdoor pattern. For example, the attacker may build a \textit{problematic} pattern that if a user's age is larger than 50 and gender is female then the credit card application would be approved; this pattern may cause the super client lose money. 

If there are some countermeasures to alleviate this possible attack, for example, compute the correlation coefficient between each feature and the label and eliminate those obvious features (e.g., high correlated), the attacker can also use more sophisticated method to bypass this kind of examination. 

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-problem.tex <==
\section{Problem Statement}\label{sec:problem-statement}
%In this section, we first present the system model and threat model in Section \ref{subsec:problem:system-model} and \ref{subsec:problem:threat-model}, respectively. 
%
%Then we present our inference attack problem on predictions in vertical FL in Section \ref{subsec:problem:vfl-prediction}.\par

\subsection{System Model}\label{subsec:problem:system-model}
We consider a set of $m$ distributed parties (or data owners) $\{P_1, \cdots, P_m\}$ who train a vertical FL model by consolidating their respective datasets. 
%
After obtaining the trained vertical FL model parameters $\boldsymbol{\theta}$, the parties collaboratively make predictions on their joint prediction dataset $\mathcal{D}_{\text{pred}}=\{D_1, \cdots, D_m\}$.
%
Each row in the dataset corresponds to a sample, and each column corresponds to a feature. 
%
Let $n$ be the number of samples and $d_i$ be the number of features in ${D}_i$, where $i \in \{1, \cdots, m\}$. 
%
We denote $D_i = \{\boldsymbol{x}_{i}^{t}\}_{t=1}^{n}$ where $\boldsymbol{x}_{i}^{t}$ represents the $t$-th sample of $D_i$. 
%Let $Y = \{y_t\}_{t=1}^n$ be the set of sample labels. 
%
In this paper, we consider the supervised classification task and denote the number of classes by $c$.
%
Table \ref{table:notations} summarizes the frequently used notations. 
\par

In vertical FL, the datasets $\{{D}_1, \cdots, D_m\}$ share the same sample ids but with disjoint subsets of features \cite{YangLCT19}. 
%
In particular, we assume that the parties have determined and aligned their common samples using private set intersection techniques \cite{Pinkas0SZ15, ChenLR17} without revealing any information about samples not in the intersection. 
%
%In addition, we assume that the label set $Y$ is only held by the active party.

\subsection{Threat Model}\label{subsec:problem:threat-model}

We consider the semi-honest model \cite{Mohassel17, WuWZLCL18, ChowdhuryW0MJ20} where every party follows the protocol exactly as specified, but may try to infer other parties' private information based on the messages received. 
%
Specifically, this paper focuses on the situation that the active party is the adversary. The active party may also collude with other passive parties to infer the private feature values of a set of target passive parties. 
%
The strongest notion is that $m-1$ parties collude (including the active party) to infer the feature values of the remaining passive party. 
%
Note that this is true when there are only two participating parties in the data collaboration.
%
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }
In addition, we assume that the active party has no background information of the passive parties' data distribution. However, he may know the passive parties' feature names, types, and value ranges; this is reasonable because the active party often needs this information to justify the effectiveness of the trained model. 
% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }

\ifthenelse{\boolean{isrevision}}
{
}
{
We do not consider malicious behaviors in this paper. On the one hand, a malicious active party who deviates from the agreed protocol will obtain inaccurate model predictions, leading to a wrong decision. The risk might be too high compared to the gain of the inferred information.
%
On the other hand, a malicious passive party who provides useless or incorrect feature values may receive no rewards and lose trust in his collaborators. For example, the active party could apply some incentive methods to justify the contributions of those provided data~\cite{simcollaborative}. 
}

\begin{table}[t]
\centering
\caption{Summary of notations}
\begin{tabular}{  l  l }
\toprule
Notation & Description \\
\toprule
$m$ & the number of parties in vertical FL \\
$n$ & the number of samples in the prediction dataset \\
$d$ & the number of total features \\
$c$ & the number of classes in the classification \\
$\boldsymbol{x}$ & an input sample in the prediction stage \\
$\boldsymbol{v}$ & the prediction output, i.e., confidence scores of $\boldsymbol{x}$ \\
${P}_{\text{adv}}$ & the adversary (the active party and several passive parties) \\
${P}_{\text{target}}$ & the attack target (the remaining passive parties) \\
${d}_{\text{adv}}$ & the number of features hold by ${P}_{\text{adv}}$ \\
${d}_{\text{target}}$ & the number of features hold by ${P}_{\text{target}}$ \\
${\boldsymbol{x}}_{\text{adv}}$ & the feature values of $\boldsymbol{x}$ hold by ${P}_{\text{adv}}$ \\
${\boldsymbol{x}}_{\text{target}}$ & the feature values of $\boldsymbol{x}$ hold by ${P}_{\text{target}}$ \\
%${D}_i$ & predict dataset hold by $P_i$ \\
%$d_i$ & the number of features in ${D}_i$ \\
$\boldsymbol{\theta}$ & the parameters of the trained vertical FL model \\
$\boldsymbol{\theta}_G$ & the parameters of the generator model \\
%$\boldsymbol{x}_{i}^t$ & $t$-th sample in $D_i$ \\
%$\boldsymbol{x}_{i,j}^t$ & $j$-th feature of the $t$-th sample in $D_i$ \\
%$\alpha$ & learning rate \\
%$T$ & the number of maximum iterations in training \\
%$B$ & batch of samples in mini-batch SGD algorithm \\
\bottomrule
\end{tabular}
\label{table:notations}
\end{table}

\subsection{Feature Inference Attack on Model Predictions} \label{subsec:problem:vfl-prediction}

Given the vertical FL model parameters $\boldsymbol{\theta}$, the parties can jointly make predictions on new input samples, whose feature values are distributed among $m$ parties. 
%
As described in Section \ref{subsec:background:machine-learning}, the prediction output consists of a vector of confidence scores, i.e., $\boldsymbol{v} = (v_1, \cdots, v_c)$.
%
%In vertical FL, the prediction is usually started by the active party who sends a prediction request to other parties, along with an input sample id. 
%
%Then the other parties prepare the feature values of the corresponding sample, and all parties can jointly run a secure protocol (e.g., \cite{WuCXCO20}) to compute $\boldsymbol{v}$ such that no intermediate information is disclosed except $\boldsymbol{v}$. 
%
In this paper, we assume that $\boldsymbol{\theta}$ and $\boldsymbol{v}$ are revealed to the active party because this information is essential for the active party to make correct and interpretable decisions. 
\par

Let $\boldsymbol{x}$ be an input sample for prediction. 
%
Without loss of generality, the $m$ parties can be abstracted into two parties: the adversary $P_{\text{adv}}$, which is composed of the active party and a subset of colluding passive parties; and the attack target $P_{\text{target}}$, which is composed of the remaining passive parties. 
%
Let $\boldsymbol{x} = (\boldsymbol{x}_{\text{adv}}, \boldsymbol{x}_{\text{target}})$, such that $\boldsymbol{x}_{\text{adv}}$ and $\boldsymbol{x}_{\text{target}}$ denote the feature values held by $P_{\text{adv}}$ and $P_{\text{target}}$, respectively; and $d_{\text{adv}}$ and $d_{\text{target}}$ denote the number of features held by $P_{\text{adv}}$ and $P_{\text{target}}$ accordingly.

As a consequence, the setting for our feature inference attack is as follows. The adversary $P_{\text{adv}}$ is given the vertical FL model parameters $\boldsymbol{\theta}$, the prediction output $\boldsymbol{v}$, and the feature values $\boldsymbol{x}_{\text{adv}}$ that belongs to himself. $P_{\text{adv}}$'s goal is to infer the feature values of $P_{\text{target}}$, i.e., 
%In this paper, we explore the problem that: to what extent the information of $P_{\text{target}}$'s feature values could be inferred by $P_{\text{adv}}$, i.e., 
\begin{align}
    \label{eq:attack-problem}
    \hat{\boldsymbol{x}}_{\text{target}} = \mathcal{A}(\boldsymbol{x}_{\text{adv}}, \boldsymbol{v}, \boldsymbol{\theta})
\end{align}
where $\hat{\boldsymbol{x}}_{\text{target}}$ is the inferred feature values and $\mathcal{A}$ is an attack algorithm executed by $P_{\text{adv}}$. 
%
Specifically, we use two metrics to evaluate the attack performance. 
%
One is \textit{mean square error} (MSE), measuring the deviation of the inferred feature values from the ground-truth $\boldsymbol{x}_{\text{target}}$.
% the ground-truth is a little ambiguous, people usually take it as confidence scores.
The other is \textit{correct branching rate} (CBR), which is defined for the attacks on tree-based models, measuring the fraction of inferred feature values that belong to the same branches as those computed by the ground-truth.
% correct branches in the tree models comparing to the branches computed by the ground-truth. 
A detailed discussion will be presented in Section~\ref{sec:experiments}.

==> Vertical FL Attack Draft (arXiv final)/tex-files/sec-related-work.tex <==
\section{Related Work}\label{sec:related-work}

%%%wyc: comment out on 20200916
%\textit{(1) Machine learning attacks; (2) Federated learning attacks (horizontal FL), inference attacks vs. active attacks, white-box vs. black-box, membership inference vs. property inference; (3) Vertical federated learning. }

%\noindent
%\textit{(Please skip this section as it is incomplete).} \textbf{Inference attacks.} \cite{ZhuLH19} proposes an attack using the gradients in horizontal federated learning. The attack works as follows: the attacker (could be any participating client) first randomly generates a pair of dummy inputs and labels and performs the usual forward and backward. After determining dummy gradients from the dummy data, the attacker optimizes the dummy inputs and labels to minimize the distance between dummy gradients and received real gradients. The final output is the optimized inputs and labels, which are close to the real inputs and labels. \cite{HitajAP17} proposes an attack using generative adversarial networks (GANs). The objective of the attacker is to infer meaningful information about a label that it does not own. The attacker does not compromise the central parameter server (PS) that collects and distributes parameters to the participants. The attack works as follows: the attacker trains his local GANs (unknown to the victim) to mimic class (e.g., `a') from the victim and generates samples from the GAN and labels them as class `c'. By injecting fake samples from `a' as class `c' into the distributed learning procedure. In this way, the victim needs to work harder to distinguish between class `a' and class `c' and hence will reveal more information about class `a' than initially intended. \cite{TramerZJRR16} proposes an attack to steal model from the server. The attacker has black-box access to some target model $f$ and attempts to learn a model $\hat{f}$ that closely approximates, or even matches, $f$. There are mainly three methods for initiating the attack. The first is a simple equation-solving model extraction method, which uses a number of queries (larger than the number of unknown parameters) to extract the model parameters. The second is a path-finding algorithm for extracting decision trees. These two methods use the confidence scores for the inference. The third method is an attack when the confidence scores are not revealed. They also show that the extracted model can be used to improve the accuracy of attribute inference.

%\subsection{Vertical Federated Learning}
\vspace{1mm}\noindent
\textbf{Vertical federated learning.} 
With horizontal FL being thoroughly studied~\cite{McMahanMRHA17, choudhury2020anonymizing, YangLCT19}, vertical FL is receiving increased attention, and there have been several solutions~\cite{hardy2017private, Mohassel17, OhrimenkoSFMNVC16, ChengCorr19, HuNYZ19, WuCXCO20} proposed recently. 
%
\cite{hardy2017private, ChengCorr19} apply partially homomorphic encryption \cite{Paillier99} in the LR and GBDT models to protect the information exchanged among the parties.
%
\cite{Mohassel17} and \cite{WuCXCO20} utilize secure multiparty computation to provide strong data security for the NN and tree-based models, respectively, ensuring that no intermediate information other than the final output is disclosed.
%For logistic regression, \cite{hardy2017private} proposes to approximate logistic loss with Taylor expansion, then integrate intermediate outputs from different clients by additively homomorphic encryption. \cite{cheng2019secureboost} and~\cite{WuCXCO20} both focus on tree-based models: \cite{cheng2019secureboost} employs homomorphic encryption to protect privacy, while \cite{WuCXCO20} further utilizes secure multiparty computation to enhance the functionality of models. Compared to logistic regression and tree-based models, neural networks are more difficult to be adapted to vertical FL given that simply splitting network into sub-models could severely degrade model performance.
%\cite{liu2018secure} proposes a transfer learning framework to build flexible models in different clients by leveraging rich samples without common IDs. 
%
Also, secure hardware could protect the parties' private data during the training and prediction stages using secure enclaves \cite{OhrimenkoSFMNVC16}. 
%
By allowing that the active party's labels can be shared with the passive parties, \cite{HuNYZ19} proposes a vertical FL framework, by which each party computes a prediction from a trained local model, and then the parties aggregate the local predictions into a final prediction. 
%trains a local model and then the aggregates different local predictions into a final prediction. Such methods could preserve the privacy of features whereas sacrificing the prediction accuracy. 

Nevertheless, existing vertical FL solutions focus on protecting data privacy during the training or prediction process. In this paper, we consider the most stringent case that the computation of model training and model prediction is secure enough, and the adversary only utilizes the computation output (i.e., the trained model and model predictions) to infer the attack target's private feature values. 
%these schemes, which are designed to mainly protect the privacy of training and testing data, could be vulnerable under our attacking framework, considering that few of them have defenses in prediction phase.

%\subsection{Attacks on Federated Learning}
\vspace{1mm}\noindent
\textbf{Inference attacks on federated learning.}
%Traditional ML methods need to gather and store data in a centralized server before training, thus incur great concerns over data privacy and confidentiality~\cite{li2020federated}. Federated learning (FL) is therefore proposed to solve the issue of data privacy and fragmentation~\cite{YangLCT19}. FL could be further categorized into horizontal FL and vertical FL, in which training data are split by sample and by feature respectively~\cite{YangLCT19}. 
Recent studies have demonstrated that FL is vulnerable to multiple types of inference attacks, such as \textit{membership inference}~\cite{NasrSH2019, MelisSCS19}, \textit{property inference}~\cite{MelisSCS19}, and \textit{feature inference}~\cite{hitaj2017deep, ZhuLH19, wang2019beyond}. 
%
Membership inference~\cite{NasrSH2019, MelisSCS19} aims to determine whether a specific record is in a party's training dataset or not, and the attacking effectiveness is closely related to the overfitting nature of ML algorithms~\cite{ShokriSSS17, Salem0HBF019}. 
However, this attack does not exist in vertical FL because every party knows all the training sample ids intrinsically. 
%Therefore, many regularization methods, which are proposed to prevent overfitting, could be used to greatly release the privacy leakage risks caused by membership inference~\cite{shokri2017membership, salem2018ml}. 
Property inference~\cite{MelisSCS19} attempts to extract some underlying properties or statistics of a party's training dataset, which are uncorrelated to the training task~\cite{ganju2018property, MelisSCS19}. 
%
Feature inference~\cite{hitaj2017deep, ZhuLH19, wang2019beyond} is to recover the samples used in a party's training dataset. 
%
%

Unfortunately, these inference attacks are only applicable to the training stage of horizontal FL. The reason is that they greatly rely on the iteratively exchanged gradients during the training process to build meta-classifiers for the inference. 
%
On the contrary, we focus on the feature inference in the prediction stage of vertical FL, which is more challenging because the adversary knows little information about the attack target's data. To our knowledge, this is the first work that addresses this problem. In addition, our attack methods do not depend on any intermediate information during the prediction process. 

%Gradients of global trained model, used to train meta-classifiers~\cite{NasrSH2019, MelisSCS19} or GANs~\cite{hitaj2017deep, wang2019beyond}, is indispensable in these attacking methods. Typically, in the training phase, local model gradients are shared in horizontal FL~\cite{mcmahan2017communication}, while only intermediate model outputs, instead of gradients, are shared~\cite{hardy2017private, cheng2019secureboost, HuNYZ19} in vertical FL. That is, these attacks are only applicable to horizontal FL.

%As far as known, we are the first to propose an attack framework targeting vertical FL.
%In addition, the feature inference schemes in~\cite{hitaj2017deep, wang2019beyond} are only applicable to neural works, while our framework could effectively recreate private features from logistic regression, neural network and tree-based algorithms.


%\subsection{Attacks on Machine Learning}
\vspace{1mm}\noindent
\textbf{Other related studies.}
In addition to feature inference in FL, another line of research tries to infer private feature values based on model predictions of a centralized ML model. For example, \cite{fredrikson2014privacy} proposes an attack to infer patients' genetic markers given black-box access to a linear regression model. Nevertheless, the adversary needs background information of all features except the targeting feature, making this attack relatively impractical. Similarly, the inference attack to the DT model in~\cite{fredrikson2015model} requires a marginal prior distribution for each feature, and the image reconstruction attack also relies on auxiliary information to define the cost function of the attack.
% \ifthenelse{\boolean{isrevision}}
% {
% \color{blue}
% }
In vertical FL, it is often difficult for the active party to collect prior information from the passive parties. In contrast, our attack methods do not rely on any background information of the attack target's data distribution.

The basic idea of~\cite{zhang2020secret} is similar in spirit to ours, i.e., inferring sensitive features (pixels) based on known image patches and white-box models. But this scheme requires pre-training on public images for obtaining the general image distributions, whereas our approach does not rely on the prior data distribution of the target features. Besides, \cite{zhang2020secret} aims to recover the training samples, whereas our attack methods mainly focus on reconstructing the prediction samples.
%However, these methods rely on background information for the inference, such as statistics or marginal data distribution of the unknown features. 

% \ifthenelse{\boolean{isrevision}}
% {
% \color{black}
% }
%Another line of research assumes that the adversary is malicious, i.e., he could deviate from the specified protocol for initiating the attack. 


%In~\cite{yeom2018privacy}, the effectiveness of feature inference greatly relies on overfitting and feature influence on model outputs.

%Machine learning (ML) algorithms are vulnerable to multiple types of inference attacks, such as membership inference~\cite{ShokriSSS17, Salem0HBF019, NasrSH2019}, property inference~\cite{ateniese2015hacking, ganju2018property, MelisSCS19} and feature inference (or model inversion in some literature)~\cite{fredrikson2014privacy, fredrikson2015model, yeom2018privacy, zhu2019deep}. 
%\textit{Membership inference} aims to determine whether a specific record is in the training dataset or not, and the attacking effectiveness is closely related to the inherent overfitting nature of ML algorithms~\cite{shokri2017membership, salem2018ml}. Therefore, many regularization methods, which are proposed to prevent overfitting, could be used to greatly release the privacy leakage risks caused by membership inference~\cite{shokri2017membership, salem2018ml}. \textit{Property inference} aims to learn global properties or statistics of the training dataset, considering that ML models tend to extract dataset properties which are uncorrelated to the main task~\cite{ganju2018property, MelisSCS19}. \textit{Feature inference} is used to accurately recreate samples that are used in training phase. \cite{fredrikson2014privacy} proposes a scheme to infer patients' genetic markers given black access to a linear regression model. Nevertheless, the attacker needs background knowledge of all features except the targeting feature, which makes this attack relatively weak. Similarly, inference attack to decision tree in~\cite{fredrikson2015model} needs marginal priors for each feature, and image reconstruction attack needs auxiliary information to define attacking cost function. In~\cite{yeom2018privacy}, the effectiveness of feature inference greatly relies on overfitting and feature influence on model outputs.

%Different to these feature inference attacks, our attacking framework recreates targeting features in prediction phase, which is more difficult than recreating features in training set given that trained ML models never see prediction samples before. Further, our framework could effectively recreate targeting features based only on partial features owned by attackers, and still works well without prior distribution or other auxiliary information. In addition, our attacking framework does not rely on whether the model is overfitted or not.

==> tex-files/revision.tex <==
\onecolumn

\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

\begin{auxmulticols}{2}

We would like to thank all the reviewers for their insightful and constructive comments. We have carefully addressed the comments, and have highlighted the major changes in the revised paper in {\color{blue} blue}.

\section*{Summary of Changes}
\label{sec-changes}

% \begin{itemize}
    % \item 
We have repeated the experiments relevant to Random Forest, changing the number of trees from 20 to 100, and implemented two new experiments for testing the impact of increasing query size with two real-world datasets. We added explanations and discussions on the questions raised in the review, and gave examples for each of the proposed methods.
% \end{itemize}

% \section*{Response to Meta-Reviewer}
% \noindent
% \textbf{Comment 1.} The reviewers liked the paper and would like to see a revision. Each reviewer lists a reasonably concrete list of suggestions. Please try to address them all.

% \vspace{2mm}\noindent
% \textbf{Response.} We have carefully addressed the comments point by point and revised the paper.

\section*{Response to Reviewer 1}
\noindent
\textbf{W1.} Some details of the proposed attacks need more explanations.

\noindent
\textbf{D1.} As W1 mentioned, how to approximately infer the features when $d_{target}\geq c$ in Sec.~IV-A? As most results in the experiments on equality solving attacks are in such case, please supplement the details of this part.

\vspace{2mm}\noindent
\textbf{Response.} We have refined the presentation in Section~\ref{subsec:attacks-lr-nn:specfic}. 
%
In particular, when $d_{\text{target}} \geq c$, the inference method is the same as that for $d_{\text{target}} \leq c -1$, i.e., $\hat{\boldsymbol{x}}_{\text{target}} = {\boldsymbol{\Theta}}_{\text{target}}^{+} \boldsymbol{a}$, where ${\boldsymbol{\Theta}}_{\text{target}}^{+}$ is the pseudo-inverse matrix of ${\boldsymbol{\Theta}}_{\text{target}}$. 
%
The rationale is that the solution based on the pseudo-inverse matrix not only minimizes the error norm $||\boldsymbol{\Theta}_{\text{target}} \hat{\boldsymbol{x}}_{\text{target}} - \boldsymbol{a}||_2$ but also minimizes the solution norm $||\hat{\boldsymbol{x}}_{\text{target}}||_2$, which provides a relatively good estimation, as demonstrated in our experiments. 
%
%In Section~\ref{subsec:experiments:individual}, we gave more explanations on the changes of the $\text{MSE}(\hat{\boldsymbol{x}}_{\text{target}}, \boldsymbol{x}_{\text{target}})$ under $d_{\text{target}} \geq c$.

\vspace{2mm}\noindent
\textbf{D2.} What is the time complexity of algorithm 1? Besides, what is the meaning of $\beta_{2k+1}$ and $\beta_{2k+2}$ in algorithm 1? Please clarify the details.

\vspace{2mm}\noindent
\textbf{Response.} We have added the time complexity analysis for Algorithm~\ref{alg:path-restriction}, and refined the presentation in Section~\ref{subsec:attack-dt}. 
%
The algorithm's time complexity is $O(n_f)$, where $n_f$ is the number of tree nodes in the full binary tree model. 
%
This is because the adversary needs to traverse the tree model to compute the indicator vectors for recording those tree nodes that may be evaluated in his perspective. 
%
Regarding $\beta_{2i+1}$ and $\beta_{2i+2}$ in the algorithm, they represent the corresponding indicators in $\boldsymbol{\beta}$ with respect to node $i$'s left and right child nodes, respectively. 
%
Specifically, an indicator value of 1 indicates that the node might be evaluated in this prediction in the perspective of the adversary; otherwise, the node will not be accessed (i.e., the prediction paths containing this node are impossible and can be eliminated). 

\vspace{2mm}\noindent
\textbf{W2.} The paper lacks of necessary examples to illustrate the proposed algorithms.

\noindent
\textbf{D3.} As W2 mentioned, though there is a simple example for path restriction attack, the algorithms would be more comprehensible if there are examples for the equality solving attack and attacks based on multiple predictions.

\vspace{2mm}\noindent
\textbf{Response.} As advised, to improve the presentation of the proposed attack methods, we have added two examples for the equality solving attack (Example~\ref{example:esa}) and generative regression network attack (Example~\ref{example:grna}) in Section~\ref{subsec:attacks-lr-nn:specfic} and Section~\ref{subsec:attacks-grn}, respectively.

\vspace{2mm}\noindent
\textbf{D4.} In Fig.~4, the increase of the MSE on datasets Bank marking and News popularity is much larger than that on Credit card and Drive diagnosis. In Fig.~5, the CBR of PRA increases slightly as $d_{\text{target}}$ increases, which contradicts the common sense and other instances. Please analyze the reasons.

\vspace{2mm}\noindent
\textbf{Response.} We have analyzed the reasons and added more explanations in Section~\ref{subsec:experiments:individual}. 
%
Regarding the phenomenon in Fig.~\ref{fig:esa-performance}, the root cause is from the different distributions of the four datasets. 
%
Based on the pseudo-inverse matrix inference method, we compute the upper bound of the MSE between the inferred solution $\hat{\boldsymbol{x}}_{\text{target}}$ and the ground-truth $\boldsymbol{x}_{\text{target}}$, i.e., $\text{MSE}(\hat{\boldsymbol{x}}_{\text{target}}, \boldsymbol{x}_{\text{target}})$, for the Bank, Credit, Drive, News datasets, which are 0.6, 0.14, 0.45, and 0.34, respectively. 
%
In general, a larger upper bound implies a lower attack accuracy that the adversary can achieve. This explains why the increase of the MSE on Bank is much larger than the other datasets. 
%
Besides, although the upper bound of Drive is larger than that of News, there are 11 classes for this dataset, i.e., the adversary can obtain 10 equations for the inference, which contains more information than that from News (i.e., 4 equations). Therefore, the MSE of Drive is smaller than that of News. 

In terms of the counter-intuitive CBR trend on the Drive dataset in Fig.~\ref{subfig:pra-drive}, there are two reasons. 
%
First, the Drive dataset has 11 classes, which is much more than those in other datasets (2 in Bank and Credit, 5 in News). As such, in Drive, each class corresponds to a smaller number of tree paths. 
%
Therefore, given one specific class, there exist only a small number of candidate prediction paths, which leads an improved CBR. In this case, the adversary would not gain a significant advantage by knowing more features. %may not facilitate further restrictions. 
%
Second, the decision tree model only selects informative features during training, which means that the increase of $d_{\text{target}}$ in Drive does not necessarily increase the number of unknown features in the tree, since some features may never be selected. As a consequence, a larger $d_{\text{target}}$ do not always decrease the CBR of the PRA attack. 

%First, there are more classes (11) in Drive than in other datasets (2 in Bank and Credit, 5 in News), which means in the Drive dataset, one class could correspond to less tree branches. The possible prediction paths of one specific class can be therefore greatly reduced, leading to a sufficiently good CBR. And more known features may not facilitate further restrictions. Second, the decision tree model does not include all the features. Due to the randomness of feature selection, the increase of $d_{\text{target}}$ (i.e. unknown features) does not necessarily decrease the number of known features selected in the tree model, which means larger $d_{\text{target}}$ in Drive may not decrease the CBR of the PRA attack. 

\vspace{2mm}\noindent
\textbf{D5.} What are the values of mean $\mu$ and standard deviation $\sigma$ used in the baseline random guess method? Please clarify.

\vspace{2mm}\noindent
\textbf{Response.} The mean and standard deviation of the Gaussian distribution in the random guess method are $\mu = 0.5$ and $\sigma = 0.25$, respectively. This ensures that at least 95\% of the generated samples are within $(0, 1)$. We have clarified the settings and added another random guess baseline according to the Uniform distribution $\boldsymbol{U}(0, 1)$ in Section~\ref{subsec:experiments:setup}.

\section*{Response to Reviewer 3}
\noindent
\textbf{D1.} Mitigation techniques are discussed and also evaluated to show their effects on presented attacks. However, I wonder why the authors did not at all mention differential privacy as one additional mitigation technique.

\vspace{2mm}\noindent
\textbf{Response.} We did not mention differential privacy (DP) since it is unsuitable in our setting. In particular, DP requires that any information from sensitive data should be released using a randomized function, such that even if we arbitrarily change a record in the function's input, the distribution of the function's output remains roughly the same. In our context, the sensitive data is an unlabelled record, and the function that releases information is a machine learning model that predicts the record's label. If we are to achieve DP, then we should inject noise into the model, such that even if we arbitrarily modifies the input record, the distribution of the model's output label is almost unchanged. In other words, the model should provide roughly the same prediction for any input record. This apparently renders the model useless. Therefore, DP is unsuitable for our problem. In the revised paper, we include the above discussion in Section~\ref{sec:defense}.

%Differential Privacy (DP) is employed for protecting individual's data privacy such that the probability of producing a given output is not highly dependent on whether a particular sample is included in the input dataset or not. Essentially, DP is more effective in protecting data privacy over multiple samples. However, in the prediction stage of vertical FL, the sample id should be known to all the parties, i.e., every party knows exactly the predicting sample, which does not satisfy the DP definition. In fact, how to incorporate DP into vertical FL models is still an open problem. Therefore, DP is not considered as a defense method in this paper. 
%(\textit{Is this explanation persuasive or reasonable? Do we need to add this explanation in the main text?})

\vspace{2mm}\noindent
\textbf{W2.} It is not clear why mean square error is chosen as the metric to evaluate attack performance.

\noindent
\textbf{D2.} Currently, the attack performance for ESA and GRNA is evaluated with the measurement of mean square error. According to equation (10) the effect is averaged over all features in the data set. However, I am not sure if this is the right approach for real-world scenarios: there I expect different features having different privacy levels. A brief discussion how the errors are distributed between different features would be helpful to further understand the attack's consequences. For example, target features that are strongly correlated with features the adversary knows would result in lower errors intuitively.



\vspace{2mm}\noindent
\textbf{Response.} Since the equality solving attack (ESA) and generative regression network attack (GRNA) are regression tasks, we use the mean square error (MSE) to measure their overall accuracy in reconstructing multiple target features.
We added more discussion regarding the impact of data correlation between the known features $\boldsymbol{x}_{\text{adv}}$ and the unknown features $\boldsymbol{x}_{\text{target}}$ on the attack performance in Section~\ref{subsec:experiments:multiple}. As demonstrated in Fig.~\ref{fig-corre}, we found that a stronger correlation would result in a higher attack accuracy. Therefore, in real-world scenarios, the adversary may exploit prior knowledge of attribute correlations to estimate the accuracy of his attacks. %further decide whether to believe the inferred feature values based on their correlations with the known feature values. 

\vspace{2mm}\noindent
\textbf{W1.} The evaluation with synthetic data is not very well motivated. I understand that the authors decided to use synthetic data to evaluate different numbers of predictions, however, it is not completely clear to me why this was not possible with real-world datasets (with reduced numbers in that case).

\vspace{2mm}\noindent
\textbf{Response.} As advised, we have added new experiments using two real-world datasets (i.e., Drive diagnosis and News popularity) to evaluate the impact of different query sizes on the attack performance. The results show a similar trend to those using synthetic datasets. We have updated Fig.~\ref{fig:grn-sample-size} and the corresponding descriptions in Section~\ref{subsec:experiments:multiple}.

\section*{Response to Reviewer 4}
\noindent
\textbf{D1.} The paper proposes a novel attack in the setting of vertical federated learning which has drawn significant attention recently. It begins with an intuitive logistic regression to demonstrate the feasibility of such an attack. Even though this paper focuses on federated learning, the proposed methodology is also applicable to the problem of model inversion for sensitive features such as [1]. It is necessary to compare with the approaches in those attacks and address the differences.

\noindent
[1] The Secret Revealer: Generative Model-Inversion Attacks Against Deep Neural Networks, CVPR, 2020

\vspace{2mm}\noindent
\textbf{Response.} The basic idea of [1] is similar in spirit to ours, as it also tries to infer sensitive features (i.e., pixels) based on known image patches and white-box models. However, the method in [1] has two major differences from our approach. First, the method in [1] requires pre-training on public images to obtain the general image distributions, whereas our approach does not rely on the prior data distribution of the target features. Second, [1] aims to recover the training samples, whereas our attack methods mainly focus on reconstructing the prediction samples. We have added discussions on [1] in Section~\ref{sec:related-work}.

\vspace{2mm}\noindent
\textbf{D2.} The threat model can be improved. The paper claims that their method requires no background information while the definition of “background” is not clear. If it includes everything even the name/type of those features, it makes the inferred results less threatening given that the attacker has no idea what those features represent.

\vspace{2mm}\noindent
\textbf{Response.} We have improved the presentation of the threat model in Section~\ref{subsec:problem:threat-model} and the corresponding descriptions in Sections~\ref{sec:introduction} and \ref{sec:related-work}. Specifically, we emphasize that the adversary does not have background information of the attack target's data distribution, but may know the unknown feature's name, type, and value range. This assumption is reasonable because, in practice, the active party in vertical federated learning often needs this information to explain and justify the trained model before deploying it into the production system. 

\vspace{2mm}\noindent
\textbf{D3.} In Section V, the paper develops multiple predictions attack based on the assumption that the candidate tree combinations are large and 100 trees can produce (40,100), approximately $1\times{10}^{28}$. However, in the evaluation, the maximum number of trees is 20 which makes it only (8,20) combinations, which is around $1\times{10}^{5}$. It will be more sensible to have the same number of trees as the assumption does.

\vspace{2mm}\noindent
\textbf{Response.} We have conducted new experiments using 100 trees for the random forest model and updated Fig.~\ref{fig:grna-performance} and Fig.~\ref{fig:grna-rf-performance-cbr}. The results are similar to the setting with 20 trees, which demonstrates the effectiveness of the proposed attack method. We have also revised the description of this setting in Section~\ref{subsec:experiments:setup}.

\vspace{2mm}\noindent
\textbf{D4.} In Fig.~3, it seems building the generative model with a random input $\boldsymbol{r}^t$ is not meaningful since it neither contributes to the back-propagation or is necessarily needed as a seed.

\vspace{2mm}\noindent
\textbf{Response.} We have added the explanation of the effect of random input $\boldsymbol{r}^t$ in Section~\ref{sec:attack-multiple-predictions}. In fact, the random vector $\boldsymbol{r}^t$ is an indispensable component of GRN. First, it acts as a regularizer, encouraging the generator to capture more randomness arising from $\boldsymbol{x}^t_{\text{adv}}$. Second, in different epochs, the $\boldsymbol{x}^t_{\text{adv}}$ of a specific sample can be concatenated with different $\boldsymbol{r}^t$ into different generator inputs, which derive various gradient directions during the back-propagation and thus lead to a better estimation of $\boldsymbol{x}^t_{\text{target}}$ with high probabilities. 
In the experiments, we found that a generator with random inputs can reduce the reconstruction error by $20\%$ compared to those without random inputs.
Due to space limitation, we include this set of experiments in the arXiv version of this paper. 

\vspace{2mm}\noindent
\textbf{D5.} The impact of query size is important to the problem of multiple predictions since they need to be done by multiple parties jointly in vertical federated learning, which is missing from the evaluation or discussion.

\vspace{2mm}\noindent
\textbf{Response.} The impact of query size, i.e., the number of predictions, is evaluated in Section~\ref{subsec:experiments:multiple}, as shown in Fig.~\ref{fig:grn-sample-size}. In the revised paper, we have added new experiments on two real-world datasets (i.e., drive diagnosis and news popularity) to illustrate its effect on the attack performance. The results show that attack accuracy could be improved when the adversary accumulates more prediction outputs, which is expected as the generator model can be trained more accurately given more predictions. We have revised the description in Section~\ref{subsec:experiments:multiple}.

\vspace{2mm}\noindent
\textbf{D6.} In Section VI, the baselines are built by random samples from Gaussian distribution without specification of mean and variance. Besides, the uniform distribution should be more suitable for a random baseline. This needs to be clarified as the samples are most likely to be drawn from the mean area in Gaussian distribution.

\vspace{2mm}\noindent
\textbf{Response.} We have clarified the Gaussian distribution setting in the experiments: the mean is 0.5 and the standard deviation is 0.25. This setting ensures that at least 95\% of the generated samples are within (0,1). In addition, we have added another random baseline with a uniform distribution $\boldsymbol{U}(0,1)$ and updated Fig.~\ref{fig:esa-performance}, Fig.~\ref{fig:grna-performance} and Fig.~\ref{fig:grn-sample-size} in Section~\ref{sec:experiments}. 
%The results show that the two random baselines achieve a similar performance, (\textit{explain the reason?}).

\vspace{2mm}\noindent
\textbf{Minors.} Page 2: using multiple prediction;
Page 11: this is the first work addresses this problem.

\vspace{2mm}\noindent
\textbf{Response.} We have corrected the mentioned grammar problems.

\end{auxmulticols}

\twocolumn

==> tex-files/sec-acknowledgements.tex <==
\section*{Acknowledgement}\label{sec:acknowledgements}

This work is supported by xxx.

==> tex-files/sec-poisoning-attacks.tex <==
\section{Poisoning Attacks}\label{sec:poisoning-attacks}

In this section, we present two kinds of data poisoning attacks: \textbf{random noise attack} and \textbf{correlated pattern attack}. The goal of the attacks is to decrease the model accuracy. Both attacks are initiated by the ordinary clients. The former attack is achieved by providing useless features with random noise, while the latter attack is achieved by providing features that are highly correlated to labels to backdoor the trained model. \par 

\subsection{Random Noise Attack}\label{subsec:random-noise-attack}

This attack injects some random noises to the local training dataset, to decrease the accuracy of the trained model. \textit{(Naive)}.

\subsection{Correlated Pattern Attack}\label{subsec:correlated-pattern-attack}

This attack assumes that the attacker has some background knowledge, i.e., a small subset (e.g., 5\%) of labels of samples in the training dataset. This assumption is reasonable in the malicious setting, for example, a business competitor of the super client may collude with an ordinary client and provide the labels of some overlapped samples in the training dataset. \par

Given the small subset of labeled samples, the attacker can train a classifier using its local features, and predict the labels of the rest of samples in the training dataset. After obtaining these labels, the attacker may modify the values of its local features to correlate to the labels, resulting in a backdoor pattern. For example, the attacker may build a \textit{problematic} pattern that if a user's age is larger than 50 and gender is female then the credit card application would be approved; this pattern may cause the super client lose money. 

If there are some countermeasures to alleviate this possible attack, for example, compute the correlation coefficient between each feature and the label and eliminate those obvious features (e.g., high correlated), the attacker can also use more sophisticated method to bypass this kind of examination. 
